KBQA: Learning Question Answering over QA Corpora and Knowledge Bases

Question answering (QA) has become a popular way for humans to access billion-scale knowledge bases. Unlike web search, QA over a knowledge base gives out accurate and concise results, provided that natural language questions can be understood and mapped precisely to structured queries over the knowledge base. The challenge, however, is that a human can ask one question in many different ways. Previous approaches have natural limits due to their representations: rule based approaches only understand a small set of "canned" questions, while keyword based or synonym based approaches cannot fully understand the questions. In this paper, we design a new kind of question representation: templates, over a billion scale knowledge base and a million scale QA corpora. For example, for questions about a city's population, we learn templates such as What's the population of $city?, How many people are there in $city?. We learned 27 million templates for 2782 intents. Based on these templates, our QA system KBQA effectively supports binary factoid questions, as well as complex questions which are composed of a series of binary factoid questions. Furthermore, we expand predicates in RDF knowledge base, which boosts the coverage of knowledge base by 57 times. Our QA system beats all other state-of-art works on both effectiveness and efficiency over QALD benchmarks.

==> Anatomy.tex <==
% !TEX root = qa2.tex

\section{Our Approach: KBQA}
\label{sec:anatomy}

In this section, we study the problem of answering binary factoid questions. In Sec~\ref{sec:anatomy:model}, we use a probabilistic model to model the QA problem. More details are illustrated in Sec~\ref{sec:anatomy:pi} and Sec~\ref{sec:anatomy:ppt}, where Sec~\ref{sec:anatomy:pi} contains the online inference, and Sec~\ref{sec:anatomy:ppt} contains the offline template learning. The offline template learning requires an entity\&value recognition procedure, which is shown in Sec~\ref{sec:noise}.



%Furthermore, the answer to the question is a simple value.

%%  one predicate, and . first introduce our
%% probabilistic inferencing model to find the value of a question from a
%% knowledge base in Sec~\ref{sec:anatomy:pi}. This inferencing need
%% $P(P|T)$. So we propose another the probabilistic model for template
%% extraction and computing $P(P|T)$ in
%% Sec~\ref{sec:anatomy:ppt}. And we present the implementations for
%% both probabilistic inferencing and template extraction in
%% Sec~\ref{sec:anatomy:qu:algorithm}.


\subsection{A Probabilistic Model}
\label{sec:anatomy:model}
Our approach KBQA learns question answering by using a QA corpus and a
knowledge base. However, due to issues such as
issues such as {\it uncertainty} (e.g. questions in the QA corpus may
be vague), {\it incompleteness} (e.g. the knowledge base is almost
always incomplete), and {\it noise} (e.g.  answers in the QA corpus
may be wrong) brought by the QA corpus and knowledge base, we create a probabilistic model for QA over knowledge base.

\begin{pdef}
\label{pdef:pvq}
Given a question $q$, our goal is
to find an answer $v$ in the knowledge base that has the maximal
probability ($v$ is a simple value):
\begin{equation}
\small
\argmax_{v}P(V=v|Q=q)
\end{equation}
\vspace{-0.5cm}
\end{pdef}

KBQA creates a probabilistic model for the above problem. This is
shown in Figure~\ref{fig:pg:online}. First, from question $q$, we
identify its entities by entity
distribution $P(e|q)$. Second, we use entities and questions to infer
templates. So we get the template distribution
$P(t|q,e)$. Third, we get predicates in the knowledge base that
correspond to these templates by the predicate distribution $P(p|t)$ learned in
Sec~\ref{sec:anatomy:ppt}. Finally, given entity $e$ and
knowledge graph predicate $p$, we get the value distribution $P(v|e,p)$. We return the value with
the maximal probability as answer.



%% To solve Problem~\ref{pdef:pvq}, KBQA uses the probabilistic graph shown in
%% Figure~\ref{fig:pg:online}. With the probabilistic graph, the inference procedure
%% is reduced to the calculation of a probability distribution conditioned on the observed data.
%% KBQA first extracts entities from the given
%% question.The probability distribution $P(E|Q)$ in Figure~\ref{fig:pg:online} accounts for this procedure. Then, KBQA generates templates from the entity and question
%% by probability distribution $P(T|Q,E)$. Next,
%% KBQA derives the corresponding predicates for these templates, using
%% the template extraction result in Sec~\ref{sec:anatomy:ppt}. This
%% is represented by probability $P(P|T)$. Finally,
%% KBQA computes the probabilities of values conditioned on $E$ and $P$, i.e., $P(V|E,P)$, and returns the
%% value with maximal probability.
%% >>>>>>> .r8913

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{figs/probabilistic_graph_online.eps}
\caption{Probabilistic Graph for $P(v|q)$}
\label{fig:pg:online} %% label for entire figure
\vspace{-0.3cm}
\end{figure}

Based on the chain rule, the probabilistic graph in
Figure~\ref{fig:pg:online} implies that we can compute $p(v|q)$ by:
{
\small
\begin{flalign}
\begin{split}
\label{eqn:pvq}
P(v|q) =  P(q)\sum_{e,p,t}[P(v|e,p)P(p|t)P(t|e,q)P(e|q)]
\end{split}
\end{flalign}
}
Since $P(q)$ is a constant for computing $P(q)$, our objective is
to find:
{
\small
\begin{equation}
\argmax_{v}\sum_{e,p,t}[P(v|e,p)P(p|t)P(t|e,q)P(e|q)]
\label{equ:argmax}
\end{equation}
}

\subsection{Probabilistic Inference}
\label{sec:anatomy:pi}
In this section, we display how we compute Eq~\ref{equ:argmax}, using a simple example of answering $q_0=${\tt When was Barack Obama born?}.

{\bf Entity distribution $P(e|q)$}
For a given question $q$, we first identify entities that appear in
$q$. The entity should meet two conditions: (a) it should be a noun
in the question; (b) it should be in the knowledge base.

We use Stanford POS Tagger~\cite{toutanova2003feature} for condition (a).
And we check if noun is an entity's name in the knowledge base for condition
(b). Usually one binary factoid question only has one entity. But if there
are multiple candidate entities $E=\{e_1,...,e_n\}$, we simply give them
equal probability in this step. And for $q_0$, we have $P(Barack\ Obama|q_0)=1$.
%Much work has been done on entity resolution in text. In this
%paper, we employ the entity identification algorithm proposed by
%Collobert et al~\cite{collobert2011deep}. \Red{Why do we use this
%  algorithm? What's its advantage compared with others?} The result is
%a set of entities $E(q)=\{e_1,e_2,...,e_n\}$, where each $e_i$ is
%associated with a probability $p(e_i|q)$.

{\bf Template distribution $P(t|q,e)$}
As we mentioned, a template is of the form {\tt When was \$person
born?}. In other words, it is a question with the mention of an
entity (e.g., ``Barack Obama'') replaced by the category of the entity
(e.g., \$person).

Let $t = t(q, e, c)$ indicate that template $t$ is obtained by
replacing entity $e$ in $q$ by $e$'s category $c$. Thus, we have
%% We do the following to obtain $P(t|q, e)$. First, we obtain the
%% category distribution of $e$  entity $e$ in question $q$, we obtain its
%% category distribution.  And since $t=q.R(\bar{e},c)$, a template's
%% probability is equal to the probability of $c$:
\begin{equation}
\small
\label{eqn:ptqe}
P(t|q, e) = P(c|q, e)
\end{equation}
where $P(c|q, e)$ is the category distribution of $e$ in the context
of question $q$. %%  $P(c|e, q^*)$ is the probability of entity $e$
%% belonging to concept $c$ in context $q^*$.
Note that an isA knowledge base such as Probase~\cite{wu2012probase}
usually gives the probability $P(c|e)$, that is, the distribution of
category giving a mention of an entity.  For example, %as shown in Table~\ref{tab:pce}, 
we may have $P(company|apple) = 0.4$,
$P(fruit|apple) = 0.6$ without context. In other words, the prior probability of
$company$ is smaller than the prior probability of $fruit$.
%\begin{table}
%\small
%\begin{center}
%\begin{tabular}{ c | c | r }
%\hline
%$e$ & $c$ & $P(c|e)$ \\ \hline
%\hline
%apple & company & 0.4 \\ \hline
%apple & fruit & 0.6 \\ \hline
%\end{tabular}
%\caption{Category Distribution of an Entity (e.g., from
%  Probase)}
%\label{tab:pce}
%\end{center}
%\vspace{-0.8cm}
%\end{table}
However, when the term ``apple'' appears in the context of a certain
question, then the distribution of $apple$'s categories may
change. For example, for question {\tt what is the headquarter
of $apple$?}, the posterior probability of $company$ may become
much higher than that of $fruit$.  
%The short text conceptualization
%method~\cite{song2011short,kim2013context} focuses on finding the category
%distribution of a mention $e$ in a context by taking into
%consideration signals such as $e$'s category distribution $P(c|e)$,
%$e$'s attribute (e.g., headquarter) distribution, $e$'s co-occurrence
%distribution, etc.
In our work, we directly apply the
conceptualization method\cite{song2011short} to find $P(c|q,e)$.  
%Table~\ref{tab:appleconceptualization} shows the resulting template distribution $P(t|e,q)$ where question $q=$ {\tt What is the headquarter of $apple$?} and entity $e =apple$.
%\begin{center}
%\small
%\begin{tabular}{ c | c }
%\hline
%$t$ & $P(t|e,q) = P(c|e,q)$ \\ \hline
%\hline
%What is the headquarter of \$company? &0.999\\ \hline
%What is the headquarter of \$fruit? &0.001 \\ \hline
%\end{tabular}
%\captionof{table}{Template Distribution through
%  ``Conceptualization''}
%\label{tab:appleconceptualization}
%\end{center}
Table~\ref{tab:pteq0} shows the resulting template distribution $P(t|q,e)$ for $q_0:$ {\tt when was Barack Obama born?} using the conceptualization technique:

\begin{center}
\small
\begin{tabular}{ c | c }
\hline
$t$ & $P(t|q_0,e) = P(c|q_0,e)$ \\ \hline
\hline
When was \$person born? &0.64\\ \hline
When was \$politician born? &0.36 \\ \hline
\end{tabular}
\captionof{table}{Template Distribution $P(t|e,q_0)$}
\label{tab:pteq0}
%\vspace{-0.2cm}
\end{center}


{\bf Predicate distribution $P(p|t)$}
In order to derive the distribution of predicates, we employ a
large QA corpus and a billion scale knowledge base. This will be
discussed in detail in Sec~\ref{sec:anatomy:ppt}.

%Suppose we have
%learned $P(p|t)$. Then, we can compute $P(p|q)$ by
%\begin{equation}
%\label{eqn:ppq}
%P(p|q)=\sum_t P(p|t)P(t|q)
%\end{equation}


As an example, let Table~\ref{tab:ppt} represent the distribution of
$P(p|t)$ learned in Sec~\ref{sec:anatomy:ppt}.

%\begin{table}[!htb]
\begin{center}
\small
\begin{tabular}{ c | c | c }
\hline
$t$ & $p$ & $P(p|t)$ \\ \hline
\hline
When was \$person born? & dob & 0.67 \\ \hline
When was \$person born? & category & 0.33 \\ \hline
When was \$politician born? & dob & 1 \\ \hline
\end{tabular}
\captionof{table}{Predicate Distribution $P(p|t)$ Learned in Sec~\ref{sec:anatomy:ppt}}
\label{tab:ppt}
\vspace{-0.2cm}
\end{center}

%We then derive $P(p|q)$ using Eq~\ref{eqn:ppq} for question
%$q={\textcircled{d}}$. The results are shown in
%Table~\ref{tab:pqp}. Since \emph{dob} has higher probability, we
%conclude the relevant predicate for question $\textcircled{d}$ is
%\emph{dob}.
%
%
%\begin{center}
%\begin{tabular}{ c | c | c }
%\hline
%$q$ & $p$ & $P(p|q)$ \\ \hline
%\hline
%${\textcircled{d}}$ & dob & 0.79 \\ \hline
%${\textcircled{d}}$ & category & 0.21 \\ \hline
%\end{tabular}
%\captionof{table}{Predicate distributtion $P(p|q)$}
%\label{tab:pqp}
%\end{center}

{\bf Value (answer) distribution $P(v|e,p)$}
For a given entity $e$ and a predicate (property) $p$ of $e$, it is
easy to find the predicate value $v$ in a knowledge base. For
example, let entity $e$ = Barack Obama, and predicate $p$ = dob. We easily get Obama's birthday, 1961, from the knowledge base. In this
case, we have $P(1961|\mbox{Barack Obama}, dob) = 1$, since Barack Obama
only has one birthday.  However, some other predicates (properties) may
have multiple values (e.g., the children of Barack Obama). In this
case, we assume equal probability for all possible values. More formalized, we compute $P(v|e,p)$ by
\begin{equation}
\label{eqn:pvep}
P(v|e,p)=\frac{|\{(e,p,v)|(e,p,v) \in \mathcal{K}\}|}{|\{(e,p,v')|(e,p,v') \in \mathcal{K}\}|}
\end{equation}

Continuing with the previous
example, we show the distribution of value $v$ of the given entity and predicate, $P(v|e,p)$, in Table~\ref{tab:pvep}.

\begin{center}
\small
\begin{tabular}{ c | c | c | c }
\hline
$e$ & $p$ & $v$ & $P(v|e,p)$ \\ \hline
\hline
Barack Obama & dob & 1961 & 1 \\ \hline
Barack Obama & category & politician & 0.5 \\ \hline
Barack Obama & category & person & 0.5 \\ \hline
\end{tabular}
\captionof{table}{Value (Answer) Distribution $P(v|e,p)$}
\label{tab:pvep}
\vspace{-0.2cm}
\end{center}

 %% More
%% formally, suppose $V(e,p)=\{v|(e,p,v) \in \mathcal{K}\}$ is the
%% satisfied value set, we have
%% \begin{equation}\label{eqn:pvep}
%% P(V=v|E=e,P=p)=\frac{1}{|V(e,p)|}.
%% \end{equation}

{\bf Putting everything together}
From the probability graph in Figure~\ref{fig:pg:online}, we can now compute the distribution of
answer value of the given question $P(v|q)$ by Eq~\ref{eqn:pvq}.

The example of $P(v|q_0)$ is shown in Table~\ref{tab:pvq}. Finally, we return $\argmax_{v}P(v|q)=1961$ to the questioner.

\begin{center}
\small
\begin{tabular}{ c | c | c }
\hline
Question & $v$ & $P(v|q_0)$ \\ \hline
\hline
${\textcircled{d}}$ & 1961 & 0.79 \\ \hline
${\textcircled{d}}$ & person & 0.11 \\ \hline
${\textcircled{d}}$ & politician & 0.11 \\ \hline
\end{tabular}
\captionof{table}{Distribution of Answer/Value $P(v|q_0)$}
\label{tab:pvq}
\end{center}
%\end{table}



%\end{example}

\subsection{Learning Question Templates}
\label{sec:anatomy:ppt}
Question templates are the internal representation that connects
natural language questions to knowledge base templates.  We have
assumed that $P(p|t)$ was given in the inference mechanism described
in the previous subsection. Now we show how to learn the
predicate distribution of given template, i.e., $P(p|t)$.

{\bf QA Corpus}
We learn templates as well as the probability distribution $P(p|t)$
from Yahoo! Answers.  Table~\ref{tab:qa} shows some real life QA pairs
in the corpus. Note that although the answer to a BFQ is
an exact value (e.g., ``1961'' for question ${\textcircled{d}}$),
answers in the QA corpus are in the form of sentences. Thus, we need to identify substring of
a sentence that corresponds to the exact value that answers the
question.

\begin{center}
\small
\begin{tabular}{ c | p{2.9cm} | p{2.9cm} }
\hline
Id & Question & Answer \\ \hline
\hline
$(q_1,a_1)$ & When was Barack Obama born? & The politician was born in 1961.\\ \hline
$(q_2,a_2)$ & When was Barack Obama born? & \reviseyq{He was born in 1961.} \\ \hline
$(q_3,a_3)$ & How many people are there in Honolulu?& It's 390K.\\ \hline
\end{tabular}
\captionof{table}{Sample QA Pairs from a QA Corpus}
\label{tab:qa}
\end{center}
%% \end{example}


{\bf A Probabilistic Model}
We compute $P(p|t)$ by
\begin{equation}
\label{eqn:pp_t}
\small
P(p|t) = \frac{P(p,t)}{P(t)}
\end{equation}
Here since $P(t)$ is a constant for computing $P(p|t)$, we only need to compute $P(p,t)$.

We compute $P(p,t)$ through the probabilistic graph in Figure~\ref{fig:pg}. First, starting from question $q$ in the graph, we find answers to $q$ by $P(a|q)$. Second, we use the qa pairs to identify the entity $e$ and value $v$. Note that in the graph, $e$ and $v$ are
associated. This is because we extract the two by $P(e,v|q,a)$ simultaneously.
We describe this process in Sec~\ref{sec:noise}. Intuitively, entity $e$ in a question and value $v$ in its
corresponding answer can determine the predicate. For instance, given $e=$ Barack Obama and $v=$
1961, a relevant predicate connecting them is ``dob''. We use $P(p|e,v)$ to represent such inference. Similar to Eq~\ref{eqn:ptqe}, we derive the template distribution from the question and entity using conceptualization by $P(t|q,e)$. As a summary of inference above, $P(p,t)$ can be computed by Eq~\ref{equ:pt}. And next we describe how to compute each component in this equation.

{
\small
\begin{flalign}
\begin{split}
P(p, t)=\sum_{q,e,v,a} P(p|e,v) P(t|q,e,v) P(e,v|q,a) P(a|q) P(q)
\end{split}
\label{equ:pt}
\end{flalign}
\vspace{-0.3cm}
}


\nop{
{\bf from here}
We compute $P(p|t)$ by:
$$P(p|t) = \frac{P(p,t)}{P(t)}$$
Since $P(t)$ is a constant for computing $P(p|t)$, we only need to compute $P(p,t)$. We have:
$$P(p, t) = \sum_{q,e,v} P(p,t|q,e,v) P(e,v|q) P(q) $$ where $q$
denotes any question in the QA corpus, $e$ denotes the entity we
identify in $q$, and $v$ denotes the value we identify in any of $q$'s
answers in the QA corpus.

When $q$, $e$, and $v$ are given, the predicate and the
template are independent. In other words, we have:
$$P(p, t) =\sum_{q,e,v} P(p|q,e,v) P(t|q,e,v) P(e,v|q) P(q)$$

Once entity and value are given, the predicate no longer depends on
the question, that is, $P(p|q,e,v) = P(q|e,v)$. Furthermore, we
introduce answers in the QA corpus as a variable into the above
equation. This finally leads to:

\begin{flalign}
\begin{split}
\small
P(p, t)=\sum_{q,e,v,a} P(p|e,v) P(t|q,e,v) P(e,v|q,a) P(a|q) P(q)
\end{split}
\label{equ:pt}
\vspace{-1cm}
\end{flalign}


The above factorization corresponds to the probabilistic graph shown
in Figure~\ref{fig:pg}. Note that in the graph, $e$ and $v$ are
associated. This is because we extract the two by $P(e,v|q,a)$ simultaneously.
We describe this process in Sec~\ref{sec:noise}.
And intuitively, entity $e$ in a question and value $v$ in its
corresponding answer can determine the predicate. For instance, given $e$ is Barack Obama and $v$
is 1961, a relevant predicate that can connect the two is ``dob'',
although there might be other predicates that can connect
the two as well.
}

%% Given the question $q$, the distribution of answer $a$ can be
%% determined by $q$. And given $q$ and $a$, we think $e$ and $v$ are
%% associated with each other. So we use a joint distribution for the
%% random variable pair $(E,V)$. The template can be generated by $q$ and
%% $e,v$. We can also obtain the predicate $p$ from $e$ and $v$ using
%% knowledge base. This graph contains $P(Q)$, $P(A|Q)$, $P(E,V|Q,A)$,
%% $P(T|Q,E,V)$, and $P(P|E,V)$. We will illustrate them below.

\begin{figure}[h]
\centering
    \includegraphics[scale=0.45]{figs/probabilistic_graph_yq2.eps}
\caption{Probabilistic Graph for $P(P|T)$}
\label{fig:pg} %% label for entire figure
\vspace{-0.3cm}
\end{figure}



{\bf Question Distribution $P(q)$ and Answer Distribution $P(a|q)$}
We assume each QA pair in the QA corpus is independent. Thus,
probability $P(a|q)$ is proportional to the frequency $a$ is provided
as an answer to question $q$. In other words, we have
\begin{equation}
\small
\label{eqn:paq}
P(a|q)=\frac{ n(q, a)}{\sum_{y} n(q, y)}
\end{equation}
where $n(q, a)$ is the frequency of pair $(q, a)$ in the QA corpus.
Similarly, we have
\begin{equation}
\small
P(q)=\frac{\sum_y n(q, y)} {\sum_{x,y} n(x, y)}
\end{equation}


As an example, consider the QA corpus in Table~\ref{tab:qa}. Note that
$q_1=q_2$. Then, we may derive the distributions of $P(q)$ and
$P(a|q)$ as follows:
\begin{center}
\small
\begin{tabular}{ c | c | c | c }
\hline
$q$ & $a$ & $P(q)$ & $P(a|q)$ \\ \hline
\hline
$q_1$ & $a_1$ & $2/3$ & $0.5$ \\ \hline
$q_2$ & $a_2$ & $2/3$ & $0.5$ \\ \hline
$q_3$ & $a_3$ & $1/3$ & $1$ \\ \hline
\end{tabular}
\captionof{table}{Distribution of Question ($P(q)$) and Answer ($P(a|q)$)}
\label{tab:q}
\end{center}

{\bf Enity\&Value Distribution $P(e,v|q,a)$}
We parse entity and value from a QA pair to derive $P(e,v|q,a)$. This
process is not trivial, especially when entities and their predicate
values come from a web scale, open domain knowledge base. Instead of
parsing them separately, we propose a joint inference approach based
on the coherence of entities and values. We will discuss this in more
detail in Sec~\ref{sec:noise}.
%
%As an example, let Table~\ref{tab:pevqa} represent the distribution of $P(e,v|q,a)$ learned in Sec~\ref{sec:noise}, where all entity\&value are correctly recognized.
%
%\begin{center}
%\begin{tabular}{ c | c  | c | c }
%\hline
%$q$ & $a$ & $e,v$ & $P(e,v|q,a)$ \\ \hline
%\hline
%$q_1$ & $a_1$ & Barack Obama , 1961 & 1 \\ \hline
%$q_2$ & $a_2$ & Barack Obama , 1961 & 1\\ \hline
%$q_3$ & $a_3$ & Honolulu, 390K & 1\\ \hline
%\end{tabular}
%\captionof{table}{Entity\&Value Distribution $P(e,v|q,a)$}
%\label{tab:pevqa}
%\end{center}


{\bf Predicate Distribution $P(p|e,v)$}
%$P(p|e,v)$ is the probability of $p$ of given $e$ and $v$ in a knowledge base. Given $e$ and $v$, there are multiple predicates connecting them in the knowledge. A simple approach is to assume that predicates of each entity have uniform distribution.
In order to compute $P(p|e,v)$, we generate all $(e, v)$ pairs from QA
pairs, and then compute $P(p|e,v)$ by
%\begin{equation}
%P(p|e,v)= \frac{P(e,v, p)}{P(e,v)} = \frac{P(v|e, p)P(p|e)P(e)}{P(e,v)} = \alpha P(v|e, p)P(p|e)
%\end{equation}

{
\small
\begin{flalign}
\begin{split}
P(p|e,v)&= \frac{P(e,v, p)}{P(e,v)} = \frac{P(v|e, p)P(p|e)P(e)}{P(e,v)} \\
&= \alpha P(v|e, p)P(p|e)
\end{split}
\end{flalign}
}

,where $\alpha$ is used to normalize the probability.
%The joint distribution $P(e,v,p)$  is derived as follows:
%\begin{flalign}
%\begin{split}
%\label{eqn:ppev}
%P(e, v, p) = P(v|e,p)P(p|e)P(e)
%\end{split}
%\end{flalign}

We have derived $P(v|e,p)$ previously in Sec~\ref{sec:anatomy:pi}. For
$P(p|e)$, we assume that predicates of any entity
have uniform distribution:
\begin{equation}
\label{equ:pplineev}
P(p|e,v)=\beta P(v|e, p)
\end{equation}
, where $\beta$ is independent from $p$ and used to normalize the probability.
Take $P(p|Barack\ Obama, 1961)$ as an example. Based on
Eq~\ref{equ:pplineev}, we compute $P(1961|Barack\ Obama,p)$.  It is
clear that only predicate $p=``dob''$ makes the probability non-zero. So
eventually we get $P(dob|Barack\ Obama,1961) =1$.

{\bf Template Distribution $P(t|q,e,v)$}
A template is generated by replacing an entity in the question with
its category.  Therefore, similar to what we described in
Eq~\ref{eqn:ptqe} in Sec~\ref{sec:anatomy:pi} , we
have:
\begin{equation}
\small
P(t|q,e,v)=P(c|e,q)
\end{equation}
Note that $P(t|q,e,v)$ is actually independent from $v$. This is
because we generate a template directly by $t=t(q,e,c)$, that is,
replacing $e$ in $q$ with $c$, without using $v$.

\textbf{Noise Tolerance} Finally, we show that our learning procedure is noise tolerant. The reason is it aggregates all qa pairs of a certain template. The aggregation guarantees that our system finds the correct predicate if \textbf{most} qa pairs of the template support the correct predicate. We also highlight that we used overall 41 million QA pairs for the training. The abundant training data guarantees that the resulting templates were trained sufficiently.
More formally, due to Eq~\ref{eqn:pp_t} and Eq~\ref{equ:pt}, we compute $P(p|t)$ by

{
\small

\begin{flalign}
\vspace{-0.2cm}
P(p|t) \propto  \sum_{(q,a),e,v} P(p|e,v) P(t|q,e,v) P(e,v|q,a) P(q,a)
\end{flalign}
}
, which sums over all qa pairs. As a result, only the predicate supported by most qa pairs will be selected, which enables our system
to tolerate with noises in the QA corpus.

%
%We now analyze the joint probability of $E$ and $V$. That is, we parse entity from the question, value from the answer, and compute their co-occurrence probability.
%
%Generally, we only need to parse entities that occurred in the question. So we define the candidate entity set $E_c(q,a)$ as:
%\begin{equation}
%\label{eqn:ecq}
%E_{c}(q,a)=\{e| \bar{e} \subset q\}.
%\end{equation}
%
%And we consider all substrings in answer as candidate values. So we define the candidate value set $V_c(q,a)$ as:
%\begin{equation}
%V_c(q,a)=\{v|v \subset a\}.
%\end{equation}
%
%But finding correct entity and value from $E_c(q,a)$ and $V_c(q,a)$ is not easy. We face several challenges:
%\begin{itemize}
%\item \emph{Parsing entity in question is not easy.} Current entity detection approaches are usually developed for one specific domain and cannot perform well on other domains~\cite{poibeau2001proper}. The problem is more striking when a large scale open domain knowledge base is used. Because, more entity candidates can be found in such a knowledge base. As an example, for the question ``When was Barack Obama born?'', we know that ``Barack Obama'' is a person and is the unique named entity in the question. But (1) ``Barack Obama'' can also be a name of a book in real knowledge base and (2) ``born'' can also be an entity in real knowledge base (a town in the Netherlands). So we need to propose a better approach that can improve the accuracy of entity detection in QA corpora.
%\item \emph{Parsing value in answer is not easy.} Answers in the QA corpora is always a long and complete sentence. Thus many noisy items are in the answer although they are not the value. For example, $a_1$ in Table~\ref{tab:qa} is a complete sentence, that many words other than ``1961'' are also in the sentence.
%%\item \emph{Capturing the correlation between entity and value is not easy.} The entity in the question and the value in the answer are correlated. We need to propose an approach that captures such correlation. Continue the previous example, suppose the answer ``1961'' is in the QA corpora. The knowledge base (as shown in Figure~\ref{fig:barackobama}) tells us that ``1961'' is exactly the birth date of node $a$ (denoting Barack Obama). In contrast, we can not find any connection between ``1961'' and ``born'' from the knowledge base.
%\end{itemize}
%
%%To solve these challenges, we propose a bipartite graph model.
%
%To solve these challenges, we proposed a new approach. Instead of parsing entity and value separately, we consider the probability of $E$ and $V$ as a joint distribution and compute their probability using their coherence. Our intuition is, the more coherence that a $(e,v)$ pair has, the more probability they are the correct entity and value. And we can use knowledge base to compute the coherence between entities and values.
%
%Note that RDF knowledge base exactly represent the relations between subject and object by $(s,p,o)$. So if $\exists (e,p,v) \in \mathcal{K}$, we say $e$ and $v$ are coherent in the knowledge base. Therefore we define the coherence of $e$ and $v$ by:
%
%\begin{equation}
%\label{eqn:co}
%co(e,v)=|\{(e,p,v)|(e,p,v) \in \mathcal{K} \}|.
%\end{equation}
%
%We define the probability of a $(e,v)$ pair is proportional to their coherence, i.e.:
%\begin{equation}
%P(E=e,V=v|Q=q,A=a)=\frac{co(e,v)}{\sum_{e' \in E_c(q,a), v' \in V_c(q,a)}co(e',v')}.
%\end{equation}
%
%\begin{example}
%Consider the problem of parsing entity and value for $(q_1,a_1)$ using knowledge base in Figure~\ref{fig:barackobama}. The only candidate entity here is $a$ ($\bar{a}=$Barack Obama).
%Due to Eq.~(\ref{eqn:co}), only two candidate values are meaningful here: $polician$ and $1961$. And we can get their coherence by the knowledge base: $co(a,polician)=corr(a,1961)=1$. The probability distribution of $P(E,V|Q,A)$ is shown in Table~\ref{tab:qaevp}. Note that here $polician$ is a noisy value. We will show how to filter it and make $P(E=Barack\ Obama,V=1961|Q=q_1,A=a_1)=1$ in Sec~\ref{sec:noise:value}.
%\end{example}
%
%\begin{center}
%\begin{tabular}{ c | c | c | c | c}
%\hline
%question & answer & entity & value & probability \\ \hline
%\hline
%$q_1$ & $a_1$ & Barack Obama & 1961 & 0.5 \\ \hline
%$q_1$ & $a_1$ & Barack Obama & polician & 0.5 \\ \hline
%\end{tabular}
%\captionof{table}{$P(E,V|Q=q_1,A=a_1)$}
%\label{tab:qaevp}
%\end{center}

%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.5]{figs/correlationGraph.eps}
%\label{fig:correlationgraph} %% label for entire figure
%\end{figure}

%%{\bf Probability $P(V|E,A)$}
%\subsubsection{Probability $P(V|E,A)$}
%Now the only unknown probability in the probabilistic graph is $P(V|E,A)$. Here answer is given, so the value must be a substring of the answer. And since the value and the entity \reviseyq{have} some relationship, we should be able to find such relationship from the knowledge base. Now we only consider simple relationship such as \emph{date of birth}. For these relationships, there should be a predicate $p$ that $(e,p,v) \in \mathcal{K}$. For more complicated relationships which cannot be represented as a simple predicate, such as the \emph{spouse} relationship in Figure~\ref{fig:barackobama}, we can get similar constraint and similar result, which will be illustrated in Sec~\ref{sec:expansion} later. \reviseyq{Thus,} given entity $e$ and answer $a$, we denote all candidate values $v$ satisfying $v$ is a substring of $a$ and $\exists p, (e,p,v) \in \mathcal{K}$ as $V(e,a)$. Therefore
%
%\begin{equation}
%\label{eqn:vea}
%V(e,a)=\{v|v \in a, \exists p, (e,p,v) \in \mathcal{K}\}.
%\end{equation}
%
%We give all values $v \in V(e,a)$ uniform probability. \reviseyq{Thus,}  we have %\reviseyq{FIX THIS EQ.}
%
%\begin{equation}
%\label{eqn:pvea}
%P(V=v|E=e,A=a)=\frac{1}{|V(e,a)|},v \in V(e,a).
%\end{equation}
%
%%\begin{subnumcases}
%%{P(V=v|E=e,A=a)=\label{eqn:pvea}}
%%\frac{1}{|V(e,a)|}, & $v \in V(e,a)$ \\
%%0, & otherwise.
%%\end{subnumcases}
%
%
%
%\begin{example}
%\label{exam:pvea}
%Consider $(q_1,a_1)$ and $(q_2,a_2)$ in Table~\ref{tab:qa}. For both questions, the entity is Barack Obama (node $a$ in Figure~\ref{fig:barackobama}). Since $V(e,a)$ are all candidate values satisfying $v$ is a substring of $a$ and $\exists p, (e,p,v) \in \mathcal{K}$, we have $V(Barack\ Obama,a_1)=\{1961,politician\}$ and $V(Barack\ Obama,a_2)=\{1961\}$.
%%Note that $V(Barack\ Obama,a_1)=\{1961,politician\}$ contains a noise value $politician$ which is not the question asking about.
%By Eq.~(\ref{eqn:pvea}), we can compute the probability \reviseyq{distribution} $P(V|E=Barack\ Obama,A=answer)$, shown in Table~\ref{tab:pvea}.
%
%\begin{center}
%\begin{tabular}{ c | c | c }
%\hline
%$A$ & $V$  &  Probability \\ \hline
%$a_1$ & 1961 & 0.5 \\ \hline
%$a_1$ & politician & 0.5 \\ \hline
%$a_2$ & 1961 & 1 \\ \hline
%\end{tabular}
%\captionof{table}{$P(V|E=Barack\ Obama,A)$}
%\label{tab:pvea}
%\end{center}
%
%\end{example}

%% %{\bf Probability $P(P|T)$}
%% \subsubsection{Probability $P(P|T)$}
%% Thus finally all probability distributions in the probabilistic graph are clear. So we can compute $P(P|T)$ by:
%% \begin{flalign}
%% \small
%% \begin{split}
%% &P(P|T) = \frac{P(P,T)}{P(T)} \propto P(P,T) \\
%% %=&\sum_q P(P,T|Q=q) P(Q=q) \\
%% %=&\sum_{q,e,v} P(P,T|Q=q,E=e,V=v) P(E=e,V=v|Q=q) P(Q=q) \\
%% %=&\sum_{q,e,v} P(P|Q=q,E=e,V=v) P(T|Q=q,E=e,V=v) \\&P(E=e,V=v|Q=q) P(Q=q) \\
%% %=&\sum_{q,e,v} P(P|E=e,V=v) P(T|Q=q,E=e,V=v) \\&P(E=e,V=v|Q=q) P(Q=q) \\
%% =&\sum_{q,e,v,a} [P(P|E=e,V=v) P(T|Q=q,E=e,V=v) \\&P(E=e,V=v|Q=q,A=a) P(A=a|Q=q) P(Q=q)].
%% \end{split}
%% \end{flalign}

%This method sometimes involves noise when computing $V(e,a)$ in Eq.~(\ref{eqn:vea}). For example, in Example~\ref{exam:pvea}, $V(Barack\ Obama,a_1)$ has a noise item: \emph{politician}. We will show how to refine this method, in Sec~\ref{sec:noise:value}.

%
%
%
%
%&P(p|t) \\
%&= \frac{P(p,t)}{P(t)} \\
%&\propto P(p,t) \\
%&= \sum_q{P(t|q)P(p,q)} \\
%&= \sum_{q,e,v}{P(t|q)P(p|v,e)P(v,e,q)} \\
%&= \sum_{q,e,v,a}{P(t|q)P(p|v,e)P(v,e|a)P(a,q)}
%\end{proof}

%
%So here, we can extract the values in the answer and compute the value distribtion, i.e., $P(v|a,e)$. Suppose the extracted values are $V(a,e)$, we give the values uniform probability:
%\begin{subnumcases}
%{P(v|a,e)=\label{eqn:pvea}}
%\frac{1}{|V(a,e)|}, & $v \in V(a,e), e=e(q(a))$ \\
%0, & otherwise.
%\end{subnumcases}
%One problem left is how to compute $V(a)$. All substrings in the answer are candidate values. To determine whether a substring is a value, we use the knowledge base. Here, since the entity in question is $e$, if $\exists p, (e,p,v) \in \mathcal{K}$ and $v$ is a substring of $a$, we will consider it as one value that the question asking about. Therefore, given $a$ and $e=e(q(a))$,
%\begin{equation}
%\label{eqn:va}
%V(a)= \{v|\exists p, (e,p,v) \in \mathcal{K}\}
%\end{equation}
%. This method sometimes involves noise. So we will show how to get more accurate $V$, in Sec~\ref{sec:noise:value}.


%Here, $P(a,q)$ denotes the probability of the co-occurrence of answer $a$, and question $q$. This can be observed by existing QA corpora. We show this more formally in Equation~\ref{eqn:paq}:
%
%\begin{subnumcases}
%{P(a,q)=\label{eqn:paq}}
%\frac{1}{\arrowvert \mathcal{QA} \arrowvert}, &$(q,a) \in \mathcal{QA}$\\
%0, &otherwise
%\end{subnumcases}

\subsection{Implementation}
\label{sec:anatomy:qu:algorithm}

As we mentioned, template learning is an offline process that
generates the $P(p|t)$ distribution, while question answering is an
online process that computes $P(v|q)$. In this section, we give some
implementation details of the two processes.

\nop{{\bf A naive method} From Eq~\ref{eqn:pvq}, it is easy to see
  that a straightforward approach for online QA is through enumerating
  all possible entities, templates, predicates, and values (exact
  answers). Thus, the complexity is $O(|E|\cdot |T|\cdot |P|\cdot
  |V|)$, where $E$, $T$, $P$, and $V$ stand for the set of all
  possible entities, templates, predicates, and values
  respectively. In the same spirit, a straightforward approach for the
  offline process of computing $P(p|t)$ based on Eq~\ref{equ:pt} can
  be achieved with a complexity of $O(|P|\cdot |T|\cdot |Q|\cdot
  |E|\cdot |V|\cdot |A|)$, where $Q$ and $A$ are the sets of questions
  and answers in the QA corpora.}

%We first give a straight forward algorithm according to Eq.~\ref{eqn:pvq} and Eq.~\ref{eqn:ppt}. We will show this algorithm is of high complexity, which motivates us to propose an improved algorithm to speedup the computation. We will show the new algorithm is of almost linear time complexity for offline procedure and almost constant time complexity for online procedure.
%
%\begin{algorithm}[h]
%\small
%  \caption{Straight Forward Algorithm}
%\begin{algorithmic}[1]
%   \Procedure {Offline}{}
%        \ForAll {$p,t,q,e,v,a$}
%                \State {Compute:\vspace{-0.1in}
%                \begin{equation}
%                \begin{array}{ll}
%                &  P(P=p|T=t) +=  \\
%                & \indent P(P=p|E=e,V=v) P(V=v|E=e,A=a) \\
%                & \indent P(E=e|Q=q) P(A=a|Q=q)  \\
%                & \indent P(T=t|Q=q) P(Q=q)
%                \end{array}\vspace{-0.1in}
%                \end{equation}}
%        \EndFor
%    \EndProcedure
%    \Statex
%    \Function {Online}{$q_{new}$}
%        \ForAll {$v,e,p,t$}
%                \State {Compute:\vspace{-0.1in}
%                \begin{equation}
%                \begin{array}{ll}
%                &  P(v|Q=q_{new}) += \\
%                & \indent P(V=v|E=e,P=p)P(P=p|T=t) \\
%                & \indent P(T=t|Q=q_{new})P(E=e|Q=q_{new})
%                \end{array}\vspace{-0.1in}
%                \end{equation}
%                }
%        \EndFor
%        \State {\Return {$\argmax_v{P(v|q_{new})}$}}
%    \EndFunction
%\end{algorithmic}
%\label{alg:naive}
%\end{algorithm}
%
%We first give the straight forward algorithm in Algorithm~\ref{alg:naive}.
%There are two major steps: (i) computing $P(P|T)$ as an offline procedure, and (ii) using Eq.~(\ref{eqn:pvq}) to compute $P(V|Q=q_{new})$ as an online procedure.
%The time complexity is shown in Theorem~\ref{th:nn}.
%\begin{theorem}
%As the procedure shown in Algorithm ~\ref{alg:naive}, the time complexity is $O(|P||T||E||V||QA|^2)$ for offline computation and $O(|P||T||E||V|)$ for online computation.
%\label{th:nn}
%\end{theorem}

\nop{{\bf A more efficient method}
The naive method is straightforward, but too expensive to
compute. They make many meaningless enumerations with zero
probabilities. For example, in the offline process, when question $q$
is given, we only need to enumerate $a$ satisfying $(q,a) \in
\mathcal{QA}$. This motivates us to find a proper order of
enumeration. In our approach, we use nodes' topological order in the
probabilistic graphs of Figure~\ref{fig:pg:online} and~\ref{fig:pg}
for enumeration.}

%We consider two factors: (1) we only need to enumerate positive probabilities. (2) We can select a proper enumeration order to make sure all the enumerated probabilities are positive. Luckily, we can use the topological order of the probabilistic graphs in Figure~\ref{fig:pg:online} and Figure~\ref{fig:pg} for the online and offline processes, respectively.

%More specifically,
For online question answering, we use the topological order of
Figure~\ref{fig:pg:online}: $question\rightarrow entity\rightarrow
template\rightarrow predicate$ $\rightarrow value$. That is, for a
question given by the user, we enumerate all entities in the
question. Then, for each entity, we enumerate its categories to obtain
all templates. For each template, we enumerate predicates $p$
satisfying $P(p|t)>0$. Finally, for entities and predicates, we
enumerate pairs that satisfy $P(v|e,p)>0$.

%% \begin{flalign}
%% \small
%% \label{eqn:online}
%% \begin{split}
%% &P(v|q) = \sum_{e \in E(q)} \sum_{c \in C(e)} \sum_{p \in P(t=T(q,e,c))} \sum_{v \in V(e,p)} \\
%% &[ P(v|e,p) P(p|t) P(t|q)P(e|q)].
%% \end{split}
%% \end{flalign}

For offline template learning, the topological order is
$question\rightarrow  answer\rightarrow entity, value \rightarrow
template \rightarrow$ $predicate$. We enumerate all QA pairs because only
these pairs satisfy $P(a|q)>0$ based on Eq~\ref{eqn:paq}. Then, for
each QA pair, we enumerate all candidate entities and values. We
further enumerate categories of each entity to get all
templates. Based on Eq~\ref{equ:pplineev}, we only need to enumerate
predicates that satisfy $P(p|e,v)>0$.

%% %The algorithm details are shown in Algorithm~\ref{alg:ala}.
%% \begin{flalign}
%% \small
%% \label{eqn:offline}
%% \begin{split}
%% &P(p|t) =  \sum_{(q,a) \in \mathcal{QA}} \sum_{(e,v) \in E_c(q,a) \times V_c(q,a)} \sum_{c \in C(e)} \sum_{p \in P(t=T(q,e,c))} \\
%% &[P(p|e,v)P(t|q,e,v) P(e,v|q,a)P(a|q)P(q)].
%% \end{split}
%% \end{flalign}


{\bf Offline Complexity} Let us first consider the time cost for each
QA pair. Suppose the average length of a QA pair is $n$ (number of
tokens). The extraction of entities and values takes $O(n)$
time. There are a few candidate entities (usually 1) in the question. So we
treat the number of entities as a constant. Then we enumerate all
concepts of each entity to generate all its templates. We also treat
the number of concepts for each entity as a constant. Each time we are
given an entity and value pair, we search their corresponding
predicates. Since there are only a few connection ways (usually 1) between them, we treat the number of such predicates as
constant. Thus the time complexity of the offline process is
$O({n}|\mathcal{QA}|)$.

{\bf Online Complexity} The time complexity analysis for the online
process is similar to that of the offline process. For one question,
it only takes linear time, i.e., $O({n})$.

%for each QA pair, we consider these factors as
%constants: the number of candidate entities for a question, the number
%of candidate values in the answer, the number of categories for each
%entity, and the number of predicates for a template.  Thus, the time
%complexity of
%complexity of the offline process is $O(|\mathcal{QA}|)$. We will
%verify this in Sec~\ref{sec:exp:efficiency} with real life data.

%In online computation, we consider these factors as constants: the number
%of entities in the question $q$, the number of categories of each
%entity, and the number of values for an entity, predicate pair.  So we
%focus on $|P(t)|$ for complexity. In the enumeration process, we carry
%out the summation $O(|\mathcal{QA}|)$ times. Each time the summation
%changes at most one $P(p|t)$ from zero to a positive value. Since
%there are $O(|T|)$ templates, the average number of $p$ that satisfies
%$P(p|t)>0$ for a given $t$ is $O(|\mathcal{QA}|/|T|)$. Thus, the time
%complexity of the online process is $O(|\mathcal{QA}|/|T|)$.  We will
%also verify this in Sec~\ref{sec:exp:efficiency}.

%Based on this intuition, we select the enumeration order: QA pair $\rightarrow$ entity $\rightarrow$ value $\rightarrow$ template $\rightarrow$ predicate. This is because the enumeration of latter variables can be controlled by former enumerated variables to avoid zero-probability. The details of this speedup algorithm is shown in Algorithm~\ref{alg:ala}. This algorithm has linear time complexity with respect to the size of QA corpora for offline procedure and almost constant time complexity for the online procedure. We conclude the equivalence between the two algorithms in Theorem~\ref{theo:alatime} and prove the reduced time complexity in Theorem~\ref{theo:same}. For detailed proof of the Theorems, please refer to the Appendix.
%\begin{theorem}
%\label{theo:same}
%$P(P|T)$ and $P(V|Q=q_{new})$ computed by the offline procedure of Algorithm~\ref{alg:naive} and Algorithm~\ref{alg:ala} are the same.
%\end{theorem}
%\begin{algorithm}[h]
%\small
%  \caption{Speedup Algorithm}
%\begin{algorithmic}[1]
%    \Function {Online}{$q_{new}$}
%        \ForAll {$e \in E(q_{new})$}
%            \ForAll {$c \in C(e)$}
%                \State {$t=q_{new}.R(\bar{e},c)$}
%                \ForAll {$p, P(P=p|T=t)>0$ \label{line:ppt:online}}
%                    \ForAll {$v, (e,p,v) \in \mathcal{K}$}
%                    \State {
%                    Compute:\vspace{-0.1in}
%                        \begin{equation}
%                        \begin{array}{ll}
%                        & \indent P(V=v|Q=q_{new}) += \\
%                        & \indent P(V=v|E=e,P=p)P(P=p|T=t) \\
%                        & \indent P(T=t|Q=q_{new})P(E=e|Q=q_{new})
%                        \end{array}\vspace{-0.1in}
%                        \end{equation}
%                    }
%                    \EndFor
%                \EndFor
%            \EndFor
%        \EndFor
%        \State {\Return {$\argmax_v{P(v|q_{new})}$}}
%    \EndFunction
%    \Statex
%    \Procedure {Offline}{}
%        \ForAll {$(q,a) \in \mathcal{QA}$}
%            \ForAll {$(e,v) \in E_c(q,a) \times V_c(q,a)$}
%                \ForAll {$c \in C(e)$}
%                    \State {$t=q.R(\bar{e},c)$}
%                    \ForAll {$p, (e,p,v) \in \mathcal{K}$}
%                        \State {\label{line:ppt:offline} Compute:\vspace{-0.1in}
%                        \begin{equation}
%                        \begin{array}{ll}
%                        & \indent P(P=p|T=t) += \\
%                        & \indent P(P=p|E=e,V=v) P(T=t|Q=q,E=e,V=v)\\
%                        & \indent P(E=e,V=v|Q=q,A=a) P(A=a|Q=q) P(Q=q)
%                        \end{array}\vspace{-0.1in}
%                        \end{equation}}
%                    \EndFor
%                \EndFor
%            \EndFor
%        \EndFor
%    \EndProcedure
%
%\end{algorithmic}
%\label{alg:ala}
%\end{algorithm}

%
%\begin{theorem}
%\label{theo:alatime}
%The complexity of Algorithm~\ref{alg:ala}, is $O(|\mathcal{QA}|(\overline{L(q,a)}+\overline{|E(q,a)||V(q,a)||C(e)|}))$ for offline computation and $O(|C||V|)$  for online computation in the worst case, and $O(|\mathcal{QA}|(\overline{L(q,a)}+\overline{V(a)})$ for offline computation and $O(\overline{|C(e)|} \overline{|V(e,p)|} \overline{|V(a)|} \frac{|\mathcal{QA}|}{|T|})$ for online computation in average cases. Here $\overline{L(q,a)}$ is the average length of the QA pair. %Here $\alpha=\overline{|V(a)|}$ and $\beta=\overline{|C(e)|} \overline{|V(e,p)|}|\overline{|V(a)|}$.
%\end{theorem}
%\begin{proof}
%For the offline procedure, we need to scan all the qa pairs. Thus we need $O(|\mathcal{QA}|\overline{L(q,a)})$ time to scan the QA corpora. For each $v \in V(a)$, we need constant time to process it. Therefore, the overall time complexity of the offline procedure is $O(|\mathcal{QA}|\overline{L(q,a)}+\overline{V(a)})$.
%
%For the online procedure in the worst case, it's easy to proof the time complexity is $O(|C||V|)$ due to the algorithm.
%For the online procedure of average cases, we need to consider the number of $p$ which has $P(p|t(q,c)) >0$. The probability $P(p|t)$ is computed by the offline procedure. Over the offline procedure, the algorithm will run line 7 $O(|QA|\overline{|V(a)|})$ times. Each time it makes at most one $P(p|t)$ from zero to positive. Since there are $O(|T|)$ templates, the average number of $p$ which has $P(p|t) >0$ for given $t$ is $O(|QA|\overline{|V(a)|}/|T|)$. Therefore we can proof the overall time complexity of the online procedure is $O(\overline{|C(e)|} \overline{|V(e,p)|} \overline{|V(a)|} \frac{|\mathcal{QA}|}{|T|})$.
%
%\end{proof}




%\begin{flalign*}
%\begin{split}
%&\therefore P(V|Q=q_{new}) =P(V|E=e(q_{new}),P)P(P|T)P(T|Q=q_{new})\\
%&P(E=e(q_{new})|Q=q_{new})
%\end{split}
%\end{flalign*}

%Through Equation~\ref{eqn:ptq}, we only need to consider $t$ satisfying $\exists c \in C(e(q_new)), t=t(q_new,c)$, because the rest values are all zero.
%
%\begin{flalign*}
%\begin{split}
%&\therefore P(V|Q=q_{new}) =\sum_{i,\exists c \in C(e(q_new)), t_i=t(q_new,c)} P(V|E=e(q_{new}),P)\\ &P(P|T=t_i)P(T=t_i|Q=q_{new})P(E=e(q_{new})|Q=q_{new})
%\end{split}
%\end{flalign*}
%
%$$\because P(v|q_{new})=\sum_{e,p,t}{P(e,t|q_{new})P(p|t)P(v|e,p)}$$
%Through equation~\ref{eqn:petq0}, we only need to consider $e=e(q_{new})$. So we have
%$$P(v|q_{new})=\sum_{p,t}{P(t|q_{new})P(p|t)P(v|e(q_{new}),p)}$$
%Through equation~\ref{eqn:petq0}, we only need to consider $t(q,c)$ for $c \in C(e(q_{new}))$. So we have
%
%\begin{flalign*}
%\begin{split}
%&P(v|q_{new}) \\
%&=\sum_{p,t}{P(t|q_{new})P(p|t)P(v|e(q_{new}),p)} \\
%&=\sum_{p,c \in C(e(q_{new}))}{P(t(q,c)|q_{new})P(p|t(q,c))P(v|e(q_{new}),p)}
%\end{split}
%\end{flalign*}
%\end{proof}

%Using Theorem~\ref{theo:ppt2} and Theorem~\ref{theo_:pvq0}, we can have the improved algorithm in Algorithm~\ref{alg:ala}.






%As shown in the experiment part (shown in Table~\ref{tab:factor_offline} and Table~\ref{tab:factor_online}), all the factors including $\overline{L(q,a)}$, $\overline{|C(e)|}$, $\overline{|V(e,p)|}$, $\overline{|V(a)|}$, and $|\mathcal{QA}|/|T|$ are small constants.
%This suggests that Algorithm~\ref{alg:ala} has linear time complexity with respect to the size of QA corpora, i.e., $|\mathcal{QA}|\overline{L(q,a)}$ for the offline procedure, and almost constant time complexity for the online procedure.


%The numbers are calculated based on the real world data set shown in this paper's experiments.}
%
%\begin{itemize}
%\item $\overline{L(q,a)}=481$. This is the average length of a qa pair.
%\item $\overline{|C(e)|}=2.3$. This is the average category number of all the entities in the knowledge base.
%\item $\overline{|V(e,p)|}=3.69$. Most predicates $p$ and entities have only one to one relations, like ``date of birth''. For these $p$, $\overline{|V(e,p)|}=1$.
%\item $\overline{|V(a)|}=0.08$. This shows less than 8\% of the answers have values (note that some answers may contain multiple values).
%The answers  without value are neither binary factoid question, nor is the binary relation in the knowledge base.
%\item $|\mathcal{QA}|/|T|=1.51$. This show that usually we do not have a template $t$ with many different questions $q$ from $\mathcal{QA}$.
%\end{itemize}

%From the these figures, we find that the complexity of the offline procedure is only
%$$|\mathcal{QA}|(\overline{L(q,a)}+\overline{V(a)})=100.02\%|\mathcal{QA}|\overline{L(q,a)}$$, and $O(\overline{|C(e)|} \overline{|V(e,p)|} \overline{|V(a)|} \frac{|\mathcal{QA}|}{|T|})=1.02$.

%So Algorithm~\ref{alg:ala} takes almost linear time about the QA corpora for offline procedure, and almost constant time for online procedure in average cases.


%\nop{
%\textbf{}\\\\\\\\\\\\\\\\\\ \textbf{new old version}
%
%The idea is to calculate the probability $P(p|q_{new})$ using the existing data: knowledge base and QA corpora. Since it's hard to compute it in a single step, our approach converts it into a multi-step process using marginal probability. It use conditional probability to compute it step by step. In each step, we can compute the conditional probability.
%
%\textbf{How people answer a question? First, people will convert the question into a template, therefore he/she can give answer for this question. To make the answer more readable, people always do not give the value directly, but use a sentence as answer to illustrate it. The value is in the answer.}
%
%\textbf{This probability of this model is hard to solve, especially for the large scale data. To compute this probability, we make an assumption, which fit our intuition for most cases: the single value will not be related to multiple predicates. More formally, $\forall v_1 \neq v_2, p, P(v_1|p)>0 \Rightarrow P(v_2|p)=0$}
%
%More specific, we use five stages to compute $P(p|q_{new})$:
%
%\begin{itemize}
%\item Stage 0: \emph{question} from user's input. We calculate the original probability $P(p|q_{new})$.
%\item Stage 1: Convert \emph{question} to \emph{template}. We think semantic of a user question $q_{new}$ should be equal to the semantic of $q_{new}$'s templates. Therefore we can introduce the conditional probability $P(t|q_{new})$ to convert a question into templates. We can compute $P(t|q_{new})$ through Named Entity Recognition (NER). The NER will parse the question $q_{new}$ to find its entity $e(q_{new})$ and the concept vector $(c_1,p_1),(c_2,p_2),...,(c_n,p_n)$, where $c_i$ is the $i$-th concept of $e$ with probability $p_i$. Thus we have
%    \begin{equation}
%    \forall t=t(q,c_i), P(t|q_{new})=p_i
%    \end{equation}
%    Since the NER has been studied in many previous works, we will not go deep into it in this paper. Through this stage, we have $$P(p|q_{new}) = \sum_{t} P(p|t)P(t|q_{new})$$. Since now the only unknown item is $P(p|t)$.
%\item Stage 2: Convert \emph{template} to \emph{question in QA corpora}. We think the predicate of a template $t$ should be equal to the predicate of questions, which fit $t$. Therefore we can introduce the conditional probability $P(q|t)$ to convert a template into questions in QA corpora. $P(q|t)$ means the probability of a template $t$ that the question $q$ fits $t$ in $\mathcal{K}$. Thus we have
%    \begin{equation}
%    P(q|t)=F(q,t)/F(t)
%    \end{equation}
%    Here
%\begin{subnumcases}
%{F(q,t)=}
%|\{q|(q,a) \in QA\}|, q \propto t\\
%0, otherwise
%\end{subnumcases}
%That is, $F(q,t)$ is the frequency of questions $q$ in the QA corpora under the condition that $q \propto t$. And $F(t)=|\{q|(q,a) \in QA\, q \propto t\}|$ is the frequency of questions $q$ that $q \propto t$. This can be done by doing NER for all $\{q|(q,a) \in QA\}$. And we will give a improvement of the NER based on the specific condition in Sec~\ref{sec:noise:ner}.
%Through this stage, we have $$P(p|q_{new}) = \sum_{q,t} P(p|q) P(q|t) P(t|q_{new})$$. Since now the only unknown item is $P(p|q)$.
%\item Stage 3: Convert \emph{question in QA corpora} to \emph{answer in QA corpora}. We think the predicate of a question should be equal to the predicate of its answer. Therefore we can introduce the conditional probability $P(a|q)$ to convert a question into its answers. $P(a|q)$ means the probability of a question $q \in \mathcal{QA}$ that the answer of it is $a$. Thus we have
%    \begin{equation}
%    P(a|q) = F(a,q) /F(q)
%    \end{equation}
%    Here $F(a,q) = |\{(q,a)|(q,a) \in QA\}|$, is the frequency of such $(q,a)$ pairs in the QA corpora. And $F(q)=|\{q|\exists a, (q,a) \in QA\}$, is the frequency of such $q$ in the QA corpora.
%    Through this stage, we have $$P(p|q_{new}) = \sum_{a,q,t} P(p|a) P(a|q) P(q|t) P(t|q_{new})$$. Since now the unknown item is $P(p|a)$.
%\item Stage 4: Convert \emph{answer in QA corpora} to \emph{value} in answer. We think the predicate of an answer should be equal to the predicate of its useful values. An answer string can be very long, and contain much useless information. Only some meaningful values in it contains the predicate information. Therefore we can introduce the conditional probability $P(v|a)$  to convert an answer into values in the answer. We will illustrate how to determine whether a value $v$ is useful later in Stage 5. Suppose the useful value set is $V$, we give the values equal probability. That is, we simply use
%    \begin{equation}
%    P(v|a)=\frac{1}{|V|}
%    \end{equation}
%    In Sec~\ref{sec:noise:value}, we will show how to set a better probability distribution.
%    Through this stage, we have $$P(p|q_{new}) = \sum_{v,a,q,t} P(p|v) P(v|a) P(a|q) P(q|t) P(t|q_{new})$$. Since now the only unknown item is $P(p|v)$.
%\item Stage 5: Convert \emph{value} to \emph{predicate} in knowledge base. In this stage, we calculate the only unknown probability $P(p|v)$. It means probability of $v$ that matches predicate $p$ in the knowledge base. We show the intuition of this probability computing in Example~\ref{example:intuitation}. This example shows that, the value $v$ occurred in the answer always represents the intent of the answer. Thus the frequency of a value's predicate always measure the probability that the value represent the semantic of this predicate. Since we have the knowledge base $\mathcal{K}$ as the background, and the entity $e(q)$ in Stage 2, it's easy to count the frequency of predicate $p$ satisfying $(e(q),p,v) \in \mathcal{K}$.
%    \begin{equation}
%    \label{eqn:ppv}
%    P(p|v)=\frac{1}{|\{p|(e(p),p,v) \in \mathcal{K} \}|}
%    \end{equation}
%    This stage also answer the question of how to compute $V$ in stage 4. Since we need to guarantee $(e(q),p,v) \in \mathcal{K}$ in Equation~\ref{eqn:ppv}, only the value $v$ satisfying $\exists p, (e(q),p,v) \in \mathcal{K}$ is meaningful. So we have $V=\{v|\exists p, (e(q),p,v) \in \mathcal{K} \}$ in stage 4.
%\end{itemize}
%
%\begin{example}
%\label{example:intuitation}
%Consider the three qa pairs in Table~\ref{tab:whenwaspeopleborn}. These questions all satisfies the template ``When was \$person born?''. All of their answers contain the value \emph{1961}, which is located in the predicate \emph{date of birth} of \emph{Barack Obama}. For the third qa pair, the value \emph{Honolulu} also occurs in the answer. This is the value located in the predicate \emph{place of birth}. So there are overall three occurrence of  \emph{date of birth}, one occurrence \emph{place of birth} in the answer, and no other predicate values occurred in the answers. This is a strong evidence that we should find the answer from predicate \emph{date of birth}.
%\end{example}
%
%\begin{table}[!htb]
%\small
%\begin{center}
%\begin{tabular}{ | l | p{2.3cm} |p{1.8cm} |}
%  \hline
%  Question & Answer & Matched predicates \\ \hline
%  \hline
%  When was Barack Obama born? & \textbf{1961}. & data of birth           \\ \hline
%  When was Bill Clinton born? & Bill Clinton was born in \textbf{1946}. & date of birth\\ \hline
%  When was Barack Obama born? & He was born in \textbf{1961} in \textbf{Honolulu}. & date of birth, place of birth\\ \hline
%\end{tabular}
%\caption{QA pairs with template ``When was was \$person born''}
%\label{tab:whenwaspeopleborn}
%\end{center}
%\end{table}
%
%
%%直接做还不能动态规划，有些地方有后效性，所以在公式的某些地方做变形，把一些内容，如stage 2的entity沉下去。
%
%\begin{flalign}
%\begin{split}
%&P(p|q_{new}) \\
%&= \sum P(p|t)P(t|q_{new}) \\
%&=\sum P(p|q) P(q|t) P(t|q_{new}) \\
%&= \sum P(p|a) P(a|q) P(q|t) P(t|q_{new}) \\
%&= \sum P(p|v) P(v|a) P(a|q) P(q|t) P(t|q_{new}) \\
%\end{split}
%\end{flalign}
%
%\begin{flalign}
%\begin{split}
%&P(p|q_{new}) \\
%&= \sum P(p|t)P(t|q_{new}) \\
%&=\sum P(p|q) P(q|t) P(t|q_{new}) \\
%&= \sum P(p|a) P(e,a|q) P(q|t) P(t|q_{new}) \\
%&= \sum P(p|e,v) P(e,v|e,a) P(e,a|q) P(q|t) P(t|q_{new})
%\end{split}
%\end{flalign}
%
%For challenge 1, (i) We use $P(t|q_{new})$, i.e., we use template as the representation of the question. Therefore many un-occurred questions still can be answered if only their templates occurred. (ii) Unlike some query understanding approaches~\cite{cao2008context}, no clustering is used during the computing. So some rare templates or rare predicates, which only occur once in the QA corpora, can also be answered.
%
%{\bf Algorithm}
%Now we illustrate the algorithm for computing $P(p|q_{new})$.
%
%A straight forward method is, we compute it from Stage 0 to Stage 5.
%
%\begin{theorem}
%Given $q_{new}$, suppose from Stage 0 to Stage 5, the number of templates, questions, answers, values, predicates are $s_1$, $s_2$, $s_3$, $s_4$, $s_5$, the complexity
%\end{theorem}
%
%
%$\\\\\\\\$
%
%\textbf{old version}
%
%In knowledge base, facts are stored in $(subject,predicate,object)$ triples. And the answer value we need, is always stored in $object$. Before getting $object$, we need $subject$ and $predicate$. To understand the binary factoid question, the first task is to recognize the entity name from it. Then we can go through the inverse direction of ``name'' to allocate the entity, i.e., $subject$. Since this problem has been well-studied as NER (Named Entity Recognition) in many previous works, we will not go deep into it in this paper.
%We focus on the understanding work after finding $subject$. That is, how to find the correct $predicate$.
%%
%%Table~\ref{tab:notation} summarizes the notations we use in this paper.
%%
%%\begin{table}[!htb]
%%\begin{center}
%%\begin{tabular}{ | c | c |}
%%  \hline
%%  Notation & Description \\ \hline
%%  \hline
%%  $q$ & question. \\ \hline
%%  $a$ & answer \\ \hline
%%  $e$ & entity \\ \hline
%%  $\mathcal{K}$ & knowledge base \\ \hline
%%  $\mathcal{QA}$ & QA corpora \\ \hline
%%  $qa$ & qa pair \\ \hline
%%  $t$ & template \\ \hline
%%  $c$ & category \\ \hline
%%  $p$ & predicate \\ \hline
%%  $v$ & value \\ \hline
%%  $s$ & subject \\ \hline
%%  $o$ & object \\ \hline
%%\end{tabular}
%%\caption{Notations}
%%\label{tab:notation}
%%\end{center}
%%\end{table}
%
%\begin{pdef}[Question understanding]
%Given the knowledge base $\mathcal{K}$ and a question $q$, we seek to find the predicate $p \in \mathcal{K}_p$ which captures the the semantic of the question. More specific, we seek to find a function $f_\mathcal{K}:Q \rightarrow \mathcal{K}_p$, which takes $q$ as input, and returns $p$. $p=f_\mathcal{K}(q)$ is the predicate that captures the the semantic of the question.
%\end{pdef}
%
%For example, for the knowledge base shown in Figure~\ref{fig:barackobama}, $$f_\mathcal{K}(When\ was\ Barack\ Obama\ born) = ``date\ of\ birth''$$.
%
%To get such function, we utilize \emph{template}. We first introduce the definition of template. For simplify, we only consider that questions that is asking about one entity.
%{\bf how about the questions asking about more than one entity?}
%
%\begin{definition}[Template]
%\label{def:template}
%A \emph{template} $t$ is a question with its entity say $e$ replaced by $e$'s concept $c$.  A question $q$ {\it fits} the template $t$, denoted by $q\propto t$, if the entity $e$ in $q$ is an instance of the concept $c$ in $t$.
%\end{definition}
%
%Table~\ref{tab:profession} contains some examples of templates with concept \emph{person}. Here, we think \emph{questions with the same template should be mapped to the same predicate, no matter what specific entity it is}. More specific, the following observation hold true.
%
%\begin{observation}
%\label{assumption:identity}
%Given the knowledge base $\mathcal{K}$ and template $t$, we have
%\begin{flalign*}
%\begin{split}
%&\forall q_1,q_2, \\
%&q_1,q_2\ fit\ t \Rightarrow f_\mathcal{K}(q_1)=f_\mathcal{K}(q_2)
%\end{split}
%\end{flalign*}
%%\begin{flalign*}
%%\begin{split}
%%&P(p|e,t,\mathcal{K}) \\
%%&=\sum_{c}P(p|c, t, \mathcal{K})P(c|e).
%%\end{split}
%%\end{flalign*}
%\end{observation}
%
%An example for observation~\ref{assumption:identity} can be found in Figure~\ref{fig:barackobama}. Given the same template ``When was \$person born'', whatever the {\it person} is  ``Barack Obama'' or ``Michelle Obama'', the answer  will be the predicate ``date of birth''. This observation is true for most cases in most common knowledge bases~\cite{bollacker2008freebase,hoffart2011yago2}. Based on this observation, the problem of \emph{mapping question to predicate} can be decomposed into two steps: \emph{first mapping question to template, and then mapping template to predicate}. Because the mapping from question to template can be easily solved by NER. Hence, the QA problem will be reduced to the {\it template understanding} problem, which is defined as:
%
%\begin{pdef}[Template Understanding]
%\label{pdef:templateunderstanding}
%Given the knowledge base $\mathcal{K}$ and a template $t$, we seek to find the predicate $p \in \mathcal{K}_p$ that it is asking about. More specific, we seek to find a function $g_\mathcal{K}:T \rightarrow \mathcal{K}_p$, which takes $t$ as input, and returns $p$, $p=g_\mathcal{K}(t)$ is the predicate that $t$ is asking about.
%\end{pdef}
%
%For example, for the knowledge base shown in Figure~\ref{fig:barackobama}, $$g_\mathcal{K}(When\ was\ \$person\ born) = ``date\ of\ birth''$$.
%
%%\begin{pdef}[Template Understanding]
%%Given one question \emph{q}, its entity \emph{e}, its template \emph{t}, and one knowledge base $\mathcal{K}$, we seek to find the predicate in the knowledge base that has the most probability to be matched.
%%\begin{eqnarray*}
%%\argmax_{p}P(p|q,e,t,\mathcal{K}), pre \in \mathcal{K}
%%\end{eqnarray*}
%%Since $q \Leftrightarrow (e,t)$, we can simplify the formula as
%%\begin{eqnarray}
%%\label{eqn:p_epk}
%%\argmax_{p}P(p|e,t,\mathcal{K}), p \in \mathcal{K}
%%\end{eqnarray}
%%\end{pdef}
%
%
%%This identity is very natural to understand, and is very basic for RDF structure. For example, in Figure~\ref{fig:barackobama}, \emph{Barack Obama}, whose category is \emph{person}, has his birthday information in the predicate \emph{date of birth}. Therefore, for another person \emph{Bill Clinton}, he should also have his birthday information in the predicate \emph{date of birth}, not other predicates like \emph{birthday} or \emph{birth date}.
%
%
%
%To compute $g_\mathcal{K}()$, we cannot use traditional web doc as the source. Because web docs only have sentences, not questions. We utilize a QA corpora with 45 million qa pairs crawled from Yahoo! Answer. These questions themselves are not very informative. But they together with their answers can help a lot. Because we can join the knowledge base and QA corpora to compute it. We show our intuition using the example below:
%
%\begin{example}
%\label{example:intuitation}
%Consider the three qa pairs in Table~\ref{tab:whenwaspeopleborn}. These questions all satisfies the template ``When was \$person born?''. All of their answers contain the value \emph{1961}, which is located in the predicate \emph{date of birth} of \emph{Barack Obama}. For the third qa pair, the value \emph{Honolulu} also occurs in the answer. This is the value located in the predicate \emph{place of birth}. So there are overall three occurrence of  \emph{date of birth}, one occurrence \emph{place of birth} in the answer, and no other predicate values occurred in the answers. This is a strong evidence that we should find the answer from predicate \emph{date of birth}.
%\end{example}
%
%
%\begin{table}[!htb]
%\small
%\begin{center}
%\begin{tabular}{ | l | p{2.3cm} |p{1.8cm} |}
%  \hline
%  Question & Answer & Matched predicates \\ \hline
%  \hline
%  When was Barack Obama born? & \textbf{1961}. & data of birth           \\ \hline
%  When was Bill Clinton born? & Bill Clinton was born in \textbf{1946}. & date of birth\\ \hline
%  When was Barack Obama born? & He was born in \textbf{1961} in \textbf{Honolulu}. & date of birth, place of birth\\ \hline
%\end{tabular}
%\caption{QA pairs with template ``When was was \$person born''}
%\label{tab:whenwaspeopleborn}
%\end{center}
%\end{table}
%
%The above example implies that the frequency of a matched predicate always measures the possibility that the template is asking about this predicate. In this case, the frequency of ``date of birth'' is 3, which is higher than the frequency of ``place of birth''. Thus, it's more possible that ``date of birth'' is the right answer. Thus  we can always choose the predicate with the highest number of occurrence in the answer, as the function value of $g_\mathcal{K}()$.
%
%More formally, given a template $t$, we first need to extract all the qa pairs in which the question $q$ fits $t$. We denote the matched templates as $\mathcal{QA}(t)$. That is,
%$$\mathcal{QA}(t)=\{<q, a>|<q, a> \in \mathcal{QA}, q\propto t\}$$.
%Then for these $qa$ pairs, follow the intuition above, we use the confidence function $\mathcal{C}(t,p)$,
%$$\mathcal{C}(t,p)= \arrowvert \{<q, a>| <q, a> \in \mathcal{QA}(t), \exists e \in q, v \in a, (e,p,v) \in \mathcal{K}\} \arrowvert$$,
%i.e., the frequency of the matched templates, as its confidence. So we can always choose the predicate with the confidence, as the function value of $g_\mathcal{K}()$. More specific, we show the formula of $g_\mathcal{K}()$ below:
%
%\begin{equation}
%\label{eqn:g}
%g_\mathcal{K}(t)=\argmax_{p\in \mathcal{K}} \mathcal{C}(t,p)
%\end{equation}
%
%
%
%%Since we already have a QA corpora crawled from Yahoo! Answer, we want to learn the probability from the existing qa pairs. We want to transfer the computing of this probability to some statistics of the qa pairs. The difference from previous works is, we do not parse the template to get phrases or words from it. We directly compute the probability in the template level. Using Ovservation~\ref{assumption:identify}, we have the following theorem:
%
%%\begin{theorem}
%%\begin{flalign*}
%%\begin{split}
%%&P(pre|e,p,\mathcal{K}) \\
%%&= \sum_{c}\frac{F(pre, p, \mathcal{K}, c)}{F(pre, \mathcal{K}, c)}P(c|e)
%%\end{split}
%%\end{flalign*}
%%\end{theorem}
%
%%\begin{proof}
%%Using observation~\ref{assumption:identify},
%%\begin{flalign*}
%%\begin{split}
%%&P(pre|e,p, \mathcal{K}) \\
%%&=\sum_{c}P(pre|c,p,\mathcal{K})P(c|e) \\
%%&=\sum_{c}\frac{F(pre, c,p, \mathcal{K})}{F(c,p, \mathcal{K})}P(c|e)
%%\end{split}
%%\end{flalign*}
%%\end{proof}
%%
%%The $F(pre, c,p, \mathcal{K})$ is the frequency of qa pairs in the QA corpora, that the $pre$, $c$, $p$, $\mathcal{K}$ co-occurs. This means that over knowledge base $\mathcal{K}$, $p$ is the template of the question, $c$ is the category of the entity, and $q$ is asking about the predicate $pre$. We can scan the QA corpora. But when we are scanning question $q$, how can we know what predicate it is asking about? To answer this question, we first give an example to show our intuition.
%%
%%\begin{example}[Use Answer as Feature]
%%\label{exam:answerfeature}
%%Suppose the question is \emph{When was Barack Obama born?} and the knowledge base is Figure~\ref{fig:barackobama}. It's hard for computer to know which predicate it's asking about directly. But after using the answer as a feature, it's much easier. Suppose the answer of the this question is \emph{He was born in 1961}. Since the knowledge $(Barack\ Obama, date of birth, 1961)$ is in the knowledge base, it gives us a strong evidence that the question is asking about the predicate \emph{date of birth}.
%%\end{example}
%
%%Based on this intuition, our method is, we tried to solve the problem reversely. Instead of finding the predicate directly, we first find the value $v$ from the answer. Then if $\exists pre \in k,(e, pre, v) \in \mathcal{K}$, it gives us a strong evidence that, $pre$ is the predicate that the question is asking for. Therefore we increase the corresponding $pre$ by one. For a RDF knowledge graph, checking whether $(e, pre, v) \in \mathcal{K}$ is quite easy. So therefore we can easily count $F(pre, c, p, \mathcal{K})$.
%%
%%And counting $F(c,p, \mathcal{K})$ would be a little easier. We just need to count the frequency that over knowledge bases $\mathcal{K}$, $t$ is the template of the question, and the entity is with the category $c$.
%
%We show the specific algorithm in algorithm 1.
%
%\begin{algorithm}[h]
%   \label{alg:pupc}
%   \caption{Compute $g_\mathcal{K}()$}
%\begin{algorithmic}[1]
%\Require{$\mathcal{QA}, \mathcal{K}$;}
%\Ensure{$g_\mathcal{K}()$};
%    \For {all $(q,a) \in \mathcal{QA}$}
%        \State {Use NER to parse $e$ from $q$, and convert $q$ into $t$}
%        \If {$\exists p \in \mathcal{K}, \exists v \in a, (e,p,v) \in \mathcal{K}$} \label{line:1}
%            \State $F(t,p) ++$
%        \EndIf \label{line:2}
%    \EndFor
%    \For {all $t$}
%        \State $F_{max} \leftarrow 0$
%        \For {all $F(t,p)$}
%            \If {$F(t,p) > F_{max}$}
%                \State $F_{max} \leftarrow F(t,p)$
%                \State $g_\mathcal{K}(t) \leftarrow p$
%            \EndIf
%        \EndFor
%    \EndFor
%\end{algorithmic}
%\end{algorithm}
%
%}

%\subsection{Ontology Inference}
%
%Actually much extra knowledge can be inferred from RDF schema~\cite{decker1998query}. For example, if the \emph{parent} predicate is in the knowledge base, the hidden predicate \emph{grandparent} can also be inferred because $parent \rightarrow parent \Leftrightarrow grandparent$. And as showed in Figure~\ref{fig:barackobama}, the \emph{person} in the event \emph{marriage} is the \emph{spouse}, which is another inferred knowledge provided by the graph structure.
%
















%\nop{
%
%hahaha\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
%In this subsection, we give the problem definition of QA over structured knowledge base. We present the problem under probabilistic model. Table~\ref{tab:notation} summarizes the notations used in this paper.
%
%\begin{table}[!htb]
%\begin{center}
%\begin{tabular}{ | l | p{5.5cm} |}
%  \hline
%  Notation & Description \\ \hline
%  \hline
%  $q$ & question. \\ \hline
%  $a$ & answer \\ \hline
%  $bfq$ & binary factoid question \\ \hline
%  $e$ & entity \\ \hline
%  $r$ & relation \\ \hline
%  $t$ & template \\ \hline
%  $t_a^b$ & the template which replace $Q$'s substring from $a$-th character to $b$-th character with $\sim$ \\ \hline
%  $k$ & knowledge base \\ \hline
%  $c$ & category \\ \hline
%  $pre$ & predicate \\ \hline
%  $v$ & value \\ \hline
%  $ts$ & template sequence \\ \hline
%  $bts$ & best template sequence \\ \hline
%\end{tabular}
%\caption{Notations}
%\label{tab:notation}
%\end{center}
%\end{table}
%
%Basically, the goal of QA over knowlegebase, is to answer the user's question through knowledge base. In this paper, we build a probabilistic model for this problem. Under the probabilistic model, we give a more formal problem definition below:
%
%\begin{pdef}[QA over knowledge base]
%Given one question \emph{q} and one knowledge base \emph{k}, we seek to find the value that has the most probability to be the answer, i.e.,
%\begin{eqnarray}
%\label{eqn:a_qk}
%\argmax_{a}P(a|q,k)
%\end{eqnarray}
%\end{pdef}
%
%In this paper, we focus on the RDF knowledge base. In a RDF knowledge base, each knowledge is represented as a triple $(subject, predicate, object)$. If we use graph to represent it, it's a directed edge from $subject$ to $object$. And the label of the edge is $predicate$.
%
%Basically, given the question $q$, due to the \emph{gap} between human language and knowledge base structure, we cannot directly find the answer from knowledge base. However, the question can be mapped to several structures of the knowledge base $k$. Through these structures, we can locate the answer value in $k$. We give an example below:
%
%\begin{example}
%\label{exam:structure}
%Suppose the question is \emph{when was Barack Obama born?}, and the knowledge base is shown in Figure~\ref{fig:barackobama}. First, the entity name \emph{Barack Obama} corresponds to the structure \\ $\overrightarrow{name} Barack\ Obama$. That is, an edge with label \emph{name}, and an object with value $Barack\ Obama$. Using this information, we can find entity \emph{a} or \emph{d}. Second, with the help of conceptualization, we can know that \emph{Barack Obama} here is a person, not a book or something else. This concept information corresponds to the structure $\overrightarrow{category} person$. Therefore we can filter entity \emph{d}. Finally, the question template \emph{when was $\sim$ born?} corresponds to the structure $\overrightarrow{date of birth}$. So that we can find the answer \emph{1961}.
%\end{example}
%
%Here, structures can have different presentations. In Example~\ref{exam:structure}, the structures are with the form $\overrightarrow{A}$ or $\overrightarrow{A}B$. However, actually any structures, which can be captured by computer, can be used. We will discuss more about the structure in Sec~.
%
%So the value is equal to the knowledge base plus structures. And the structures can be find through the question. More specific, $v \Leftrightarrow (k, S)$. And substituting it into Expression~\ref{eqn:a_qk}, we get
%
%\begin{eqnarray}
%\argmax_{k,S}P(k,S|q,k)
%\end{eqnarray}
%
%Since $k$ is given, we only need to get $S$, that is
%
%\begin{eqnarray}
%\label{eqn:S_qk}
%\argmax_{S}P(S|q,k)
%\end{eqnarray}
%
%Until now, there are two main steps for us to locate the answer value. The first step is to get $S$ through $(q,k)$. The second step is to get $v$ through $(k,S)$. For the second step, it's easy to locate $v$ once we have $k$ and $S$ using Trinity. So here our core challenge is the first step. More specific, how to calculate $P(S|q,k)$.
%
%In our model, the question $q$ contains several items $i_1, i_2, i_3, ..., i_n$. The items might be explicit or implicit in the question. And each element $i_i$ corresponds to one structure, say $s_i$, in the knowledge graph. And $S=\cup s_i$. Here, we assume that $s_i$ is independent from other $s_j$. And $s_i$ only depends on $i_i$ and $k$. So we have:
%
%\begin{theorem}
%\begin{eqnarray}
%\argmax_{S}P(S|q,k)=\argmax_{(s_1,..,s_n)}\prod_i P(s_i|(i_i),k)
%\end{eqnarray}
%\end{theorem}
%\begin{proof}
%Substituting it into Expression~\ref{eqn:S_qk}, we get
%
%\begin{flalign*}
%\begin{split}
%&\argmax_{S}P(S|q,k)\\
%&=\argmax_{(s_1,..,s_n)}P((s_1,..,s_n)|q,k)\\
%&=\argmax_{(s_1,..,s_n)}P((s_1,..,s_n)|(i_1,i_2,...,i_n),k)
%\end{split}
%\end{flalign*}
%
%\begin{eqnarray}
%\argmax_{S}P(S|q,k)\\
%=\argmax_{(s_1,..,s_n)}P((s_1,..,s_n)|q,k)\\
%=\argmax_{(s_1,..,s_n)}\prod_i P(s_i|(i_1,i_2,...,i_n),k)\\
%=\argmax_{(s_1,..,s_n)}\prod_i P(s_i|(i_i),k)
%\end{eqnarray}
%\end{proof}
%
%There are many different question categories~\cite{burger2001issues}. For the concern of the construction of today's knowledge bases, which try to include common knowledge, or facts, it's suitable to answer fact-based questions over knowledge bases. Using knowledge bases, we can answer many different kinds of fact-based questions, such as ranking \emph{which country has the largest population?}, comparison \emph{which country has larger population, USA or Japan?}, and counting \emph{how many country has larger population than 100 million?}. For all those questions, the most basic and important questions is the binary factoid questions (BFQ)~\cite{agichtein2005analysis}, i.e., questions asking about one entity's binary relation. For example, \emph{what is the population of China} is asking about the \emph{population} relation of \emph{China}. And other questions are all based on the BFQ. For example, ranking, comparison, and counting are all further processed over relation value. This high light the importance of BFQ. So in this paper, we put our main focus on the BFQ. But we also show how we solve more complex questions in Sec~\ref{sec:amatomy:parser:complex}
%
%\begin{definition}[Binary Factoid Question (BFQ)]
%BF question is the question that is asking about one entity's binary relation.
%\end{definition}
%
%Thus for BFQ, the problem \emph{BFQA over knowledge base} can be defined below:
%
%\begin{pdef}[BFQA over knowledge base]
%\label{pdef:pqaoverkb}
%Given one binary factoid question $q$ and knowledge base \emph{k}, we seek to find the value that has the most probability to be the answer, i.e.,
%\begin{eqnarray}
%\label{eqn:pqaoverkb}
%\argmax_{a}P(a|q,k)
%\end{eqnarray}
%\end{pdef}
%
%\begin{definition}[structure]
%\end{definition}
%
%Now we present our method for solving Problem~\ref{pdef:pqaoverkb}. For BFQ, $a$ can be determined once the knowledge base $k$, entity $e$, and relation $r$ is given. That is, $a \Leftrightarrow (k,e,r)$. Therefore due to Formula~\ref{eqn:pqaoverkb}, we first need to find $k$, $e$, and $r$ first:
%\begin{eqnarray}
%\argmax_{k, e, r}P(k, e, r|q,k)
%\end{eqnarray}
%
%Since here the $k$ is given, we only need to get $e$ and $r$, i.e.,
%\begin{eqnarray}
%\label{eqn:1}
%\argmax_{e, r}P(e, r|q,k)
%\end{eqnarray}
%
%To solve equation~\label{eqn:1}, we need to get $P(e, r|q,k)$ first. Here, we split it into two parts:
%\begin{eqnarray}
%P(e, r|q,k)=P(r|q, k, e)P(e|q,k)
%\end{eqnarray}
%
%In this paper, we compute $P(e|q,k)$ and $P(r|q, k, e)$ separately. We call the former part, $P(e|q,k)$, the \emph{Parser}. Because the goal of it, is to parse the question and obtain entity. And we call the latter part, $P(r|q, k, e)$, the \emph{Mapper}. Because it does the mapping from natural language question to relation in knowledge base.
%
%\subsection{Comparison with previous Model}
%Model:
%Incremental
%Feature adaptive
%
%Implement:
% Corpora: QA rather than web doc.
% template rather than phrases.
%
%\subsection{Parser}
%\label{sec:amatomy:parser}
%%\emph{challenge} how to find the right entity in the knowledge base suffering the disambiguation problem. Previous methods always tried to use concept as the feature to do this. However, there are one weak points: the quality of concept information in the knowledge base might not be very good. And we have answer for each question! Due to this advantage, we .
%
%In this subsection, we present how we implement the online parser and offline parser. We first show the challenges and differences of our problem compared with tradition Named Entity Recognition (NER) problem in Sec~\ref{sec:anatomy:parser:challenge}. Then we show how we conquer these challenges using the difference, to implement the online parser and offline parser in Sec~\ref{sec:anatomy:parser:online} and Sec~\ref{sec:anatomy:parser:offline}, respectively.  We also show how we use a simple technique to parse the complex question, that enable our system answer complex question in Sec~\ref{sec:amatomy:parser:complex}.
%\subsubsection{The challenges and differences of NER over knowledge base}
%\label{sec:anatomy:parser:challenge}
%The Named Entity Recognition (NER) problem is a well-studied problem. But for NER over knowledge base, especially NER for QA over knowledge base, there are many new challenges and differences. We list them here
%
%\begin{itemize}
% \item[challenges 1] \emph{NER over knowledge base is knowledge base depedent.} Here, it's not only the question $q$ is given, also the knowledge base $k$. Note that, the $k$ is also necessary for parsing entity. Because our goal for parsing entity, is to find the value through the relation of this entity. Since different knowledge bases can have different ontologies, we may need to parse different entities for different knowledge base. We give a simple example in Example~\ref{exam:dependency}.
% \item[challenges 2] \emph{Disambiguation\cite{navigli2009word}} Traditional NER only aim to parse a string from the question. However, for NER over knowledge base, this is not enough. Disambiguation is an important task in knowledge base because different entities might have the same name. This issue is even more serious in some large-scale knowledge base. We give an example of this challenge in Example~\ref{exam:disambiguation}
% \item[difference 1] For parsing the questions in QA corpora, the \emph{answer} is a crucial feature to recognize the entity. This is a very different from previous problems. We can leverage this feature.
%\end{itemize}
%
%\begin{example}[Knowledge base Dependency]
%\label{exam:dependency}
%Consider one question, \emph{What is the population in China?}. There can be different ontology for representing this knowledge. It can be entity \emph{China} and its relation \emph{population}. And it can also be entity \emph{population} and its relation \emph{in China}. It might even be entity \emph{population in China} and relation \emph{numeric}. These all depend on the knowledge base's ontology.
%\end{example}
%
%\begin{example}
%\label{exam:disambiguation}
%Suppose the question is \emph{Who is the wife of Barack Obama?} and the knowledge base is Figure~\ref{fig:barackobama}. We notice that there are two entities with name Barack Obama, entity $a$ and entity $d$. How can we know we should find entity $a$, not entity $d$?
%\end{example}
%
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.45]{barackobama.eps}
%\caption{A sample of RDF knowledge base}
%\label{fig:barackobama} %% label for entire figure
%\end{figure}
%
%\subsubsection{Online Parser}
%\label{sec:anatomy:parser:online}
%In this subsection, we illustrate the online part of how we compute $P(e|q, k)$. To illustrate our method, we first give the definition of \emph{template}.
%
%\begin{definition}[Template]
%\label{def:pattern}
%The \emph{template} of a BFQ \emph{q}, in which the entity is \emph{e}, is $q.replace(e,\sim)$. We use \emph{p} as the abbreviation of it. Furthermore, if $e$ in $q$ starts with the $a$-th question, and ends with the $b$-th question, we use $t_a^b$ to denote the template.
%\end{definition}
%
%\begin{example}
%Suppose the question $q$ is \emph{What is the population of China?}, and the entity is \emph{China}. Then the template is \emph{What is the population of $\sim$?}, or $q_{26}^{30}$.
%\end{example}
%
%Before getting the probability, we give one observation here:
%\begin{observation}
%\label{assumption:indep}
%$P(q|p)$ and $P(k|p)$ are independent.
%\end{observation}
%
%This observation fits our intuition. Because $q$ and $k$ are given by user and QA system respectively. Using Observation~\ref{assumption:indep}, we have Theorem~\ref{theorem:ptof}:
%
%\begin{theorem}
%\label{theorem:ptof}
%Given the question $q$ and knowledge base $k$, we have
%\begin{equation}
%P(e|q, k) \sim F(p, k)/F(p)
%\end{equation}
%Here $p=q.replace(e,'\sim')$.
%\end{theorem}
%\begin{proof}
%
%Due to Definition~\ref{def:template}, $t$ is bijective with $e$. Therefore we have
%\begin{flalign*}
%\begin{split}
%&P(e|q, k) \\
%&=P(p|q, k) \\
%&=P(q, k| p)P(p)/P(q, k) \\
%&\sim P(q, k| p)P(p)
%\end{split}
%\end{flalign*}
%
%Using observation~\ref{assumption:indep}, we have
%\begin{flalign*}
%\begin{split}
%&P(e|q, k) \\
%&\sim P(q|p)P(k|p)P(p)\\
%&=P(q)P(k|p) \\
%&\sim P(k|p) \\
%&=P(p|k)P(k)/P(p) \\
%&\sim P(p, k)/P(p) \\
%&=F(p, k)/F(p)
%\end{split}
%\end{flalign*}
%
%$$\therefore P(e|q, k) \sim F(p, k)/F(p)$$.
%\end{proof}
%
%\subsubsection{Offline Parser}
%\label{sec:anatomy:parser:offline}
%In this subsection, we present how we count $F(p, k)$ and $F(p)$. This is an offline work. Since we have QA corpora, we can scan the data. For each question $q$, we parse the entity to get the template. Then increase the $F(p, k)$ by 1. And for each substring $s$ in the question, we increase $F(q.replace(s,\sim))$ by 1.
%
%It looks like that we go back to the original question again: how to parse entity from the question? But we didn't. \emph{Because these questions are with answers.} Now we present how we parse the question using its answer. More specific, how we solve challenge 1 and challenge 2, using difference 1 in Sec~\label{sec:anatomy:parser:challenge}. We first give an example to show our intuition.
%
%%Note that, challenge 1 and challenge 2 actually give us the same issue: given a qa pair, how to parse the entity, through which we can find the relation of the question to get the answer value.
%
%
%\begin{example}[Use Answer as Feature]
%\label{exam:answerfeature}
%Still consider the example used in Example~\ref{exam:disambiguation}. Suppose the answer of the this question is \emph{Her name is Michelle Obama}. Since the knowledge \\ $(Barack\ Obama, spouse, Michelle\ Obama)$ is in the knowledge base. We can find entity $a$ successfully. And this method also successfully conquer challenge 1. Because entity $a$ surely contains the relation value which the question is asking for.
%\end{example}
%
%Based on this intuition, our method is, we tried to solve the problem reversely. Instead of finding the entity directly, we first find the value $v$ from the answer. Then, if $\exists$ entity $e \in q$, and a relation $r$, and $(e, r, v) \in k$, it means that the answer contains one value $v$ of entity $e$. This is a strong evidence that, the entity $e$ is the entity we are looking for. Therefore we increase the $F(p, k)$ of the corresponding template by one.
%
%Using the method above, we can count $F(p, k)$ and $F(p)$ by the algorithm below:
%
%%\begin{algorithm}[h]
%%\small
%% \caption{Count $F(p, k)$ and $F(p)$}
%%   \label{alg:fpatkb}
%%\begin{algorithmic}[1]
%%\REQUIRE{$QASet,k$;}
%%\ENSURE{$F(p,k),F(p)$};
%%    \FOR {all $(q, a) \in QASet$}
%%        \FOR {all substring $s \in q$}
%%            \STATE $F(q.replace(s,"\sim"))++$
%%        \ENDFOR
%%        \FOR {all candidate entity $e \in q$}\label{alg:fpatkb:einq}
%%            \IF {$\exists r, v, (e,r,v) \in k, v \in a$} \label{alg:fpatkb:vina}
%%                \STATE $F(q.replace(e,"\sim"),k)++$
%%            \ENDIF
%%        \ENDFOR
%%    \ENDFOR
%%    \RETURN $C$;
%%\end{algorithmic}
%%\end{algorithm}
%
%In this algorithm, we scan the QASet. In line~\ref{alg:fpatkb:einq}, we say one candidate entity $ent \in que \iff ent$ is one substring of $que$, and $ent$ is one entity in the knowledge base. This work is supported by the Entity Indexer in Sec~\ref{sec:architecture:indexer}. We will further illustrate how we decide whether $(e,r,v) \in k$ in Sec~\ref{sec:amatomy:mapper:relation}.
%
%\subsubsection{Complex Question}
%\label{sec:amatomy:parser:complex}
%In this section, we talk about the parsing for complex question.
%
%\begin{definition}[complex question]
%Questions which ask about one entity's relation's relation, or multiple hop relation.
%\end{definition}
%
%\begin{example}[complex question]
%The question \emph{What is the population of the capital of China?} is one complex question with two hops. To answer this question, we should first parse the template \emph{What is the population of $\sim$}. Then for the clause \emph{the capital of China}, we should parse the template \emph{the capital of $\sim$} and the entity \emph{China}.
%\end{example}
%
%For convenience of the illustration, we define template sequence here.
%
%\begin{definition}[Template Sequence]
%Given a complex question $q$, the Template Sequence $ps$ for it is a sequence of templates. $ps=p_1, p_2, ..., p_n$, that $\exists 0=a_0 \le a_1 \le a_2 \le ... \le a_n \le b_n \le b_{n-1} \le ... \le b_1 \le b_0=q.length-1$, that $p_i=sub(q,a_{i-1},b_{i-1})_{a_i-a_{i-1}}^{b_i-a_{i-1}}$, and $sub(que,a_n,b_n)$ is one entity in $k$.
%\end{definition}
%
%Due to the definition, for one complex question, there could be multiple template sequence. Here we seek to find the parsing templates with highest probability, or with highest goodness. For each single template $t$, we already have $P(p, k)$ to define this probability or goodness. So we define the goodness of a template sequence utilizing $P(p, k)$:
%
%\begin{definition}[Goodness for Template Sequence]
%Given the knowledge base \emph{k} and question \emph{q}, the \emph{goodness} for a template sequence $ps=pat_1, pat_2, ..., pat_n$ is $$G(k, q, ps)=\prod_{1\le i \le n} P(p_i,k)$$
%\end{definition}
%
%Now we can define the parsing problem for complex question.
%\begin{pdef}[Best Template Sequence]
%\label{pdef:bpp}
%Given one complex question \emph{q}, we seek to find the template sequence \emph{ps} for \emph{q} with highest goodness, i.e.,
%\begin{eqnarray}
%\label{eqn:pqaoverkb}
%\argmax_{ps}G(k,q,ps)
%\end{eqnarray}
%We denote this \emph{ps} as \emph{best template sequence}, or \emph{bps} for short.
%\end{pdef}
%
%To solve the Problem~\ref{pdef:bpp}, we first proof one property of this problem.
%
%\begin{theorem}
%\label{theo:bpp}
%Suppose the best template sequence for \emph{q} is $ps=p_1, p_2, ..., p_n$. Due to its definition, $\exists 0=a_0 \le a_1 \le a_2 \le ... \le a_n \le b_n \le b_{n-1} \le ... \le b_1 \le b_0=q.length-1$, \\ that $p_i=sub(q,a_{i-1},b_{i-1})_{(a_i-a_{i-1},b_i-a_{i-1})}$. We have $\forall 1 \le i \le n, ps_i=p_i, p_{i+1}, ..., p_n$ is also the best template sequence for $sub(q,a_{i-1},b_{i-1})$.
%\end{theorem}
%\begin{proof}
%Suppose $\exists i, ps'=p'_i, p'_{i+1}, ..., p'_n$ is one template sequence for $sub(q,a_{i-1},b_{i-1})$, and
%$$G(k, sub(q,a_{i-1},b_{i-1}), ps_i) < G(k, sub(que,a_{i-1},b_{i-1}), ps')$$.
%Then for the template sequence \\ $ps''=p_1, p_2, ..., p_{i-1}, p'_i, p'_{i+1}, ..., p'_n$, we have
%\begin{flalign*}
%\begin{split}
%&G(k, q, pp'') \\
%&=\prod_{1 \le j \le i-1}P(p_j, kb) G(k, q.sub(a_{i-1},b_{i-1}), ps') \\
%&> \prod_{1 \le j \le i-1}P(p_j, kb) G(k, q.sub(a_{i-1},b_{i-1}), ps_i) \\
%&=G(k, q, pp)
%\end{split}
%\end{flalign*}
%This against the definition of best template sequence. Therefore Theorem~\ref{theo:bpp} is proved.
%\end{proof}
%
%Using Theorem~\ref{theo:bpp}, we can easily design one $O(n^4)$ dynamic programming to solve Problem~\ref{pdef:bpp}. (Algorithm omitted). The time complexity of this algorithm can be further optimized using its montonicity. But since $n$ is always very small here, it's good enough to use this algorithm.
%
%\begin{algorithm}[h]
%\small
% \caption{Find Best Template Sequence}
%   \label{alg:bpp}
%\begin{algorithmic}[1]
%\Require{$q, P(p, kb)$, $k$;}
%\Ensure{$bps$;}
%    \For {$i=1;i\le q.length;i++$}
%        \For {$l1=1;i+l1-1 \le q.length;l1++$}
%            \State $G(i,i+l1-1)=0$
%            \If {$sub(q,i,i+l1-1)$ is one entity in $k$}
%                \State $G(i,i+l1-1)=1$
%            \EndIf
%            \State $follow1(i,i+l1-1)\leftarrow 0$
%            \State $follow2(i,i+l1-1)\leftarrow 0$
%            \For {$j=i;j \le i+l1-1;j++$}
%                \For {$l2=1;j+l2 \le i+l1;l2++$}
%                    \State $p=sub(que,i,i+l1-1)_{(j-i,j+l2-(i+l1))}$
%                    \State $np=sub(que,j,j+l2-1)$
%                    \If {$P(p, k)*G(j,j+l2-1) > G(i,i+l1-1)$}
%                        \State $G(i,i+l1-1)\leftarrow P(p, k)*G(j,j+l2-1)$
%                        \State $follow1(i,i+l1-1)\leftarrow j$
%                        \State $follow2(i,i+l1-1)\leftarrow j+l2-1$
%                    \EndIf
%                \EndFor
%            \EndFor
%        \EndFor
%    \EndFor
%    \State {$l \leftarrow 1,r \leftarrow q.length$}
%    \While {$follow1(l,r) \neq 0$}
%        \State $p=sub(q,l,r)_{(follow1(l,r),follow2(l,r))}$
%        \State $bpp.Append(p)$
%        \State $l=follow1(l,r)$
%        \State $r=follow2(l,r)$
%    \EndWhile
%    \Return $bps$
%\end{algorithmic}
%\end{algorithm}
%
%
%%\subsection{Index}
%%In line~\ref{alg:fpatkb:einq} of Algorithm~\ref{alg:fpatkb}, we need to find all candidate entities in $que$. So in this section, we present how we do this.
%%
%%Although entities are already in knowledge base, it's still not easy to do this job. The biggest challenge here, is the scalability. Nowadays, the number of entities in knowledge base is always very big. And as illustrated in Sec~\ref{sec:mp}, extra category information should also be stored. For example, Satori contains 214 million entity-category mappings. And the original size of entity-category data is about 8.3 GB, which is not suitable to be stored in memory directly. To solve this problem, we build a novel hash index called \emph{static hash array}.
%%
%%A good index method for this problem is to use hash table. For a classical hash table with separate chaining, each item is assigned to a bucket by the hash function $hash1()$. Each bucket is one list here. If hash collisions happen, new item will be append at the end of this list. And to reduce the memory cost, we only store the $hash2()$ value of each item, instead of storing the string of it. Here $hash2()$ is another hash function which is independent from $hash1()$. An example is showed in Figure~\ref{fig:hash:a} and Figure~\ref{fig:hash:b}.
%%
%%\begin{figure}
%%    \centering
%%    \subfigure[$hash1()$]{
%%        \label{fig:hash:a} %% label for first subfigure
%%        \includegraphics[scale=0.5]{hash_table.eps}}
%%    \subfigure[Dynamic table]{
%%        \label{fig:hash:b} %% label for second subfigure
%%        \includegraphics[scale=0.5]{hash_dynamic.eps}}
%%    \hspace{0.5in}
%%    \subfigure[Static hash array]{
%%        \label{fig:hash:c} %% label for second subfigure
%%        \includegraphics[scale=0.5]{hash_static.eps}}
%%    \caption{Hash table example}
%%    \label{fig:hash} %% label for entire figure
%%\end{figure}
%%
%%There are still much waste space there. Note that, the pointers here make the classical open hash available for dynamic inserting and deleting. However, in our demand, it's not necessary. In our system, the knowledge base is persistent. Therefore we do not need those pointers. We now show how we convert the dynamic hash table into the static hash array below:
%%
%%\begin{itemize}
%%\item After inserting all the entities into the dynamic hash table, rewrite the nodes in the table to an array, so that nodes in the same list of the table are adjacent in the array.
%%\item For each list in the dynamic hash table, build a pointer to the start element of the list in the array.
%%\end{itemize}
%%
%%For the example above, we can get the static hash array in Figure~\ref{fig:hash:c}. Note that, for static hash array, the memory cost for use part is less than the construction part. This is because we need to get the dynamic hash table first. However, the construction only need to be done once. We can write the static hash array into the disk after, so that we can reload it from disk later if we want to use it again.
%%
%%Therefore we can use static hash array to do the index work in memory.
%
%\subsection{Mapper}
%\label{sec:amatomy:mapper}
%
%In this section, we illustrate the mapping part. As mentioned in Sec~\ref{sec:anatomy:pd}, the specific work in this part, is to compute $P(r|q, k, e)$. That is, given one question $q$, one knowledge base $k$, and one entity $e$, we tried to find the relation $r$ in the knowledge base.
%
%We first present how to get a general mapper. We present its online part and offline part in Sec~\ref{sec:amatomy:mapper:online} and Sec~\ref{sec:amatomy:mapper:offline} respectively. Then, we give the most common relation we found, and how we solve it in Sec~\ref{sec:amatomy:mapper:relation}.
%
%\subsubsection{Online Mapper}
%\label{sec:amatomy:mapper:online}
%In this subsection, we show the online part of our method for computing $P(r|q, k, e)$.
%
%To compute this probability, we first give one observation by introducing category $c$ here:
%
%\begin{observation}
%\label{assumption:ontology}
%\begin{flalign*}
%\begin{split}
%&P(r|p, k, e) \\
%&=\sum_{c}P(r|p, k, c)P(c|e)
%\end{split}
%\end{flalign*}
%\end{observation}
%
%This observation is based on the ontology of the knowledge base. That is, different entities with the same category should share the same relation in the knowledge base. For example, in Figure~\ref{fig:barackobama}, \emph{Barack Obama}, whose category is \emph{person}, has his birthday information in the predicate \emph{date of birth}. Therefore, for another person \emph{Bill Clinton}, he should also have his birthday information in the predicate \emph{date of birth}, not other predicates like \emph{birthday} or \emph{birth date}.
%
%Now we give the theorem for computing $P(r|q, k, e)$:
%
%\begin{theorem}
%\begin{flalign*}
%\begin{split}
%&P(r|q, k, e) \\
%&= \sum_{c}\frac{F(r, p, k, c)}{F(p, k, c)}P(c|e)
%\end{split}
%\end{flalign*}
%\end{theorem}
%\begin{proof}
%Since $q \Leftrightarrow (p, e)$, we have
%$$P(r|q, k, e)=P(r|p, k, e)$$.
%
%Using observation~\ref{assumption:ontology},
%\begin{flalign*}
%\begin{split}
%&P(r|p, k, e) \\
%&=\sum_{c}P(r|p, k, c)P(c|e) \\
%&=\sum_{c}\frac{F(r, p, k, c)}{F(p, k, c)}P(c|e)
%\end{split}
%\end{flalign*}
%\end{proof}
%
%We count $F(r, p, k, c)$ and $F(p, k, c)$ in the Offline Mapper.
%
%\subsubsection{Offline Mapper}
%\label{sec:amatomy:mapper:offline}
%In this subsection, we present how we count $F(r, p, k, c)$ and $F(p, k, c)$. This is an offline work.
%
%The $F(r, p, k, c)$ is the frequency of qa pairs in the QA corpora, that the $r$, $p$, $k$, $c$ co-occurs. This means that over knowledge base $k$, $p$ is the template of the question, $c$ is the category of the entity, and $q$ is asking about the relation $r$. Based on a similar reason in Sec~\ref{sec:anatomy:parser:offline}, we think for the value $v$, $(e, r, v) \in k$, then it gives us a strong evidence that, $r$ is the relation that the question is asking for. For a RDF knowledge graph, checking whether $(e, r, v) \in k$ is quite easy. So therefore we count $F(r, p, k, c)$.
%
%And counting $F(p, k, c)$ would be a little easier. We just need to count the frequency that over knowledgebaes $k$, $p$ is the template of the question , and the entity is with the category $c$.
%
%We show the specific algorithm here:
%
%%\begin{algorithm}[h]
%%\small
%%   \label{alg:pupc}
%%\begin{algorithmic}[1]
%%\REQUIRE{$QASet, k$;}
%%\ENSURE{$F(r, p, k, c), F(p, k, c)$};
%%    \FOR {all $(q, a) \in QASet$}
%%        \STATE {parse $q$ to get entity $e$}
%%        \STATE $p \leftarrow q.replace(e,"\sim")$
%%        \FOR {all $e$'s categories $c$}
%%            \STATE $F(p, k, c) += P(c|e)$
%%            \FOR {all $e$'s relation $r$}
%%                \IF {$\exists v, (e,r,v) \in k, v \in a$}\label{alg:pupc_ve}
%%                    \STATE $F(r,p,k,c) += P(c|e)$
%%                \ENDIF
%%            \ENDFOR
%%        \ENDFOR
%%    \ENDFOR
%%    \RETURN $C$;
%%\end{algorithmic}
%%\end{algorithm}
%
%Now there is only one issue left: how to know if $(e,r,v) \in k$. We will further show how it in Sec~\ref{sec:amatomy:mapper:relation}.
%
%\subsubsection{Analysis for path relation}
%\label{sec:amatomy:mapper:relation}
%In this section, we solve the problem of deciding whether $(e,r,v) \in k$.
%
%Relations in RDF knowledge base can have different forms. The most basic one is direct predicate relation. As an example in Figure~\ref{fig:barackobama}, the predicate \emph{date of birth} is a relation. But a relation can be more complex. Also see Figure~\ref{fig:barackobama}. The relation \emph{spouse} is located on the path \emph{$marriage \rightarrow person \rightarrow name$}. Note that, actually \emph{path} is a more general form of direct predicate. And due to our observation of the knowledge base, path relation is most common relation in knowledge base. So in this paper, we focus on finding this relation. But other relations can also be learned through our method in Sec~\ref{sec:amatomy:mapper:online} and~\ref{sec:amatomy:mapper:offline}
%
%We know that, originally one RDF knowledge base usually only have $(subject, predicate, object)$ triples. So we define $path$ based on this:
%
%\begin{definition}[path]
%A \emph{path} is an ordered arrangement of predicates $path = (predicate_1, predicate_2, ..., predicate_n)$.
%\end{definition}
%
%For a $path= (pre_1, pre_2, ..., pre_n)$, we say $(subject, path, object) \in kb$ iff \\$\exists subject= object_0, object_1, object_2, ..., object_n=object$, that for all $1 \le i \le n$, $(object_{i-1}, pre_i, object_i) \in k$.
%
%Usually, for find all the paths for an entity, we use BFS or DFS. And note that, if we don't limit the length of the path, we will have infinite paths. So in our research, we only consider paths with length $\le 3$.
%
%After defining the $path$ and $(subject, path object) \in k$, we have already explained the entire solution for solving problem~\ref{pdef:pqaoverkb}
%
%\subsection{Detection for polysemous path relation}
%Omitted now.\\
%
%}



==> Architecture.tex <==

\section{Architecture}
\label{sec:architecture}
In this section, we give the architecture of our system. Figure~\ref{fig:framework} gives the overview of the architecture.

In section~\ref{sec:architecture:procedure}, we will illustrate the flow of our system. And one big advantage of our system is, we can supply QA over large scale knowledgebase within a very short time. So in section~\ref{sec:architecture:indexer} and section~\ref{sec:architecture:trinity}, we show how we use some level state-of-art techniques to obtain the good performance.

\begin{figure}[h]
\centering
\includegraphics[scale=0.45]{framework2.eps}
\caption{Architecture Overview}
\label{fig:framework} %% label for entire figure
\end{figure}

\subsection{Flow}
\label{sec:architecture:procedure}
First, we will briefly present the flow of the system. It mainly contains two parts: the online part and the offline part.

\paragraph*{Offline Flow} The goal of the offline part, is to obtain the pre-knowledge, including parser pre-knowledge and mapper pre-knowledge, for the online part. First, we put the knowledge graph into Trinity~\cite{shao2012managing}, and all entity information into Entity Indexer. Then, the qa pairs in the QA corpus come into offline parser. With the help of Entity Indexer and Trinity, the offline parser will parse the question to get the entity and pattern. It will also generate the parser pre-knowledge data. And all parsed qa pairs are transferred into the offline mapper. The offline mapper leverage the parsed qa pairs, and knowledge graph in Trinity, to generate the mapper pre-knowledge.
\paragraph*{Online Flow} Online part aims to answer the question within a quite short time. When a question comes through the UI, it will first come to the online parser. Using Entity Indexer and parser pre-knowledge, the online parser will find the entity in the question. Then, it will transferred the parsed question into the online mapper. The online mapper will leverage the parser pre-knowledge to find the relation in the knowledge graph for this question. And finally the mapper find the answer value from Trinity by the entity and the relation.

So far we have presented how offline procedure and online procedure work. To make the procedures efficiently, two important components are leveraged: the Entity Indexer, and Trinity. So next we will illustrate how we build these two components.

\subsection{Entity Indexer}
\label{sec:architecture:indexer}
In this subsection, we illustrate how we implement the Entity Indexer.

The entity Indexer is used to find the entity in the question. Although entities are already in knowledgebase, it's still not easy to do this job. One challenge here, is the scalability. Nowadays, the number of entities in knowledgebase is always very big. For example, Satori contains 214 million entity-category entries. And the original size of this data is about 8.3 GB, which is beyond the capability of memory. To solve this problem, we build a novel in-memory tool called \emph{static hash array}, which can index all these entries with less than 2GB memory.

A good index method for this problem is to use hash table. For a classical hash table with separate chaining, each item is assigned to a bucket by the hash function $hash1()$. Each bucket is one list here. If hash collisions happen, new item will be append at the end of this list. And to reduce the memory cost, we only store the $hash2()$ value of each item, instead of storing the string of it. Here $hash2()$ is another hash function which is independent from $hash1()$. An example is showed in Figure~\ref{fig:hash:a} and Figure~\ref{fig:hash:b}.

\begin{figure}
    \centering
    \subfigure[$hash1()$]{
        \label{fig:hash:a} %% label for first subfigure
        \includegraphics[scale=0.5]{hash_table.eps}}
    \hspace{0.2in}
    \subfigure[Dynamic table]{
        \label{fig:hash:b} %% label for second subfigure
        \includegraphics[scale=0.5]{hash_dynamic.eps}}
    \hspace{0.2in}
    \subfigure[Static hash array]{
        \label{fig:hash:c} %% label for second subfigure
        \includegraphics[scale=0.5]{hash_static.eps}}
    \caption{Hash table example}
    \label{fig:hash} %% label for entire figure
\end{figure}

There are still much waste space there. Note that, the pointers here make the classical open hash available for dynamic inserting and deleting. However, in our demand, it's not necessary. In our system, the knowledgebase is persistent. Therefore we do not need those pointers. We now show how we convert the dynamic hash table into the static hash array below:

\begin{itemize}
\item After inserting all the entities into the dynamic hash table, rewrite the nodes in the table to an array, so that nodes in the same list of the table are adjacent in the array.
\item For each list in the dynamic hash table, build a pointer to the start element of the list in the array.
\end{itemize}

For the example above, we can get the static hash array in Figure~\ref{fig:hash:c}. Note that, for static hash array, the memory cost for use part is less than the construction part. This is because we need to get the dynamic hash table first. However, the construction only need to be done once. We can write the static hash array into the disk after, so that we can reload it from disk later if we want to use it again.

Therefore we can use static hash array to do the index work in memory.

\subsection{Trinity}
\label{sec:architecture:trinity}
Omitted.


==> Noise.tex <==
% !TEX root = qa2.tex

\subsection{Entity\&Value Recognition}
\label{sec:noise}
%In this section, we present the noise reduction methods we use in the system. We present two main noise reduction approach. In Sec~\ref{sec:noise:ner}, we show how we improve the accuracy of entity detection for QA pairs. In Sec~\ref{sec:noise:value}, we present how we use question classification to optimize value extraction.
We now analyze the entity and value identification problem in Sec~\ref{sec:anatomy:ppt}. That is, we show how we parse the entity and value from the given QA pair, by giving the joint probability $P(e,v|q,a)$. We show this in Sec~\ref{sec:noise:jointprobability}. And we present how we use question classification and value classification to further optimize the recognition in Sec~\ref{sec:noise:value}.

\subsubsection{Joint Inference of Entity\&Value}
\label{sec:noise:jointprobability}

We need to recognize entities from the question, and values from the answer. This task is not easy. We face challenges from both entity recognition and value recognition:
\begin{itemize}[leftmargin=0.4cm]
\item \emph{Entity recognition} %Current entity detection approaches are usually developed for one specific domain and cannot perform well on other domains~\cite{poibeau2001proper}.
    Although the problem of entity recognition has been studied in many works~\cite{poibeau2001proper,finkel2005incorporating}, the problem is still striking when a large scale knowledge base is used. This is because a larger knowledge base has more candidate entities can be found in the question. This brings more uncertainty to the problem. %As an example, for the question ``When was Barack Obama born?'', we know that ''Barack Obama'' is a person and is the unique named entity in the question. But (1) ``Barack Obama'' can also be a name of a book in real knowledge base and (2) ``born'' can also be an entity in real knowledge base (a town in the Netherlands). So we need to propose a better approach that can improve the accuracy of entity identification for qa pair.
\item \emph{Value recognition} Answers in the QA corpora are always one or more sentence. Thus many noisy items are in answer. %For example, $a_1$ in Table~\ref{tab:qa} is a complete sentence, that many words other than ``1961'' are also in the sentence.
%\item \emph{Capturing the correlation between entity and value is not easy.} The entity in the question and the value in the answer are correlated. We need to propose an approach that captures such correlation. Continue the previous example, suppose the answer ``1961'' is in the QA corpora. The knowledge base (as shown in Figure~\ref{fig:barackobama}) tells us that ``1961'' is exactly the birth date of node $a$ (denoting Barack Obama). In contrast, we can not find any connection between ``1961'' and ``born'' from the knowledge base.
\end{itemize}

%To solve these challenges, we propose a bipartite graph model.

To solve these challenges, we proposed a {\it joint inference} approach. Instead of identifying entity $e$ and value $v$ {\it separately}, we extract the entity and value {\it simultaneously} to compute $P(e,v|q,a)$. The intuition is, {\it valid entity\&value pair has some relation in knowledge base}.
\begin{example}
\label{example:vqa}
Consider $(q_1,a_1)$ in Table~\ref{tab:qa}. The candidate entity and value set are $\{Barack\ Obama, ...\}$ and $\{politician, 1961, ...\}$, respectively. Since $(Barack\ Obama,$ $politician)$ and $(Barack\ Obama,$ $1961)$ are connected in the knowledge base, these two pairs are more trustworthy.
\end{example}
%We use the knowledge base to compute the joint probability. Our basic idea to compute the probability of an $(e, v)$ pair is using the predicate connecting $e$ and $v$ in the knowledge base.

Following this intuition, we give all entity\&value pairs connected in knowledge base equal probability. We denote these valid entity\&value pair set as $V(q,a)$, i.e.:
\begin{equation}
\small
\label{eqn:vqa}
V(q,a)=\{(e,v)|e \in q, v \in a, \exists p, (e,p,v) \in \mathcal{K}\}
\end{equation}

So we have
{
\small
\begin{subnumcases}
{P(e,v|q,a)=\label{eqn:pvea}}
\frac{1}{|V(q,a)|}, & $(e,v) \in V(q,a)$ \\
0, & otherwise.
\end{subnumcases}
\vspace{-0.2cm}
}

%\begin{equation}
%\label{eqn:co}
%q(e,v)=\sum_{(e,p^+,v) \in \mathcal{K}} \exp{(1-p^+.length)}
%\end{equation}
%
%
%We first need to measure our confidence on an candidate $(e, v)$ pair as a valid pair.
%We define the following function for this purpose:
%\begin{equation}
%\label{eqn:co}
%q(e,v)=\sum_{(e,p^+,v) \in \mathcal{K}} \exp{(1-p^+.length)}.% |\{(e,p,v)|(e,p,v) \in \mathcal{K} \}|.
%\end{equation}
%The definition is based on the following two principles.
%First, the more predicates connecting an $(e, v)$ pair, the more probable that $(e, v)$ is a valid entity-value pair. Second, the shorter the expanded predicate is the more probable $(e, v)$ is valid.
%%Therefore we define the coherence of $e$ and $v$ by:


\nop{
The coherence is negatively correlated with the length of $p^+$ since shorter $p^+$ tends to be meaningful predicate.

   Note that an RDF knowledge base exactly represents the relationships between subjects and objects by $(s,p^+,o)$.


 ex basic idea to compute the probability is  the {\it coherence} between them. Our intuition is, the entity in question and the value in answer are surely coherent, since people ask about the value entity about the value. So we think the more coherence that a $(e,v)$ pair has, the more probable that they are the correct entity and value.
}


%Based on the above definition,  the probability $P(e,v|q, a)$ to observe $e$ and $v$ given the QA pair $(q, a)$ can be defined as:
%\begin{flalign}
%\label{eqn:pevqa}
%\begin{split}
%P(e,v|q,a) =\frac{q(e,v)}{\sum_{e' \in E_c(q,a), v' \in V_c(q,a)}q(e',v')}. \\
%\end{split}
%\end{flalign}
%where $E_c(q,a)$ is the candidate entity set and $V_c(q,a)$ is candidate value set, respectively. The denominator is used for the normalization.


%
%\begin{equation}
%\label{eqn:pevqa}
%P(E=e,V=v|Q=q,A=a)=\frac{co(e,v)}{\sum_{e' \in E_c(q,a), v' \in V_c(q,a)}co(e',v')}.
%\end{equation}
%
%\begin{example} [Joint Infrence]
%\label{exam:jointprobability}
%Consider the problem of parsing entity and value for $(q_1,a_1)$ in Table~\ref{tab:qa} using knowledge base in Figure~\ref{fig:barackobama}. The only candidate entity here is $a$ with $\bar{a}=$``Barack Obama''.
%Due to Eq.~(\ref{eqn:co}), only two candidate values are meaningful here: $politician$ and $1961$. Thus we have $q(a,politician)=q(a,1961)=1$. Table~\ref{tab:qaevp} shows the probability distribution of $P(E,V|Q,A)$. Note that here $politician$ is a noisy value. We will show we filter it to make $P(E=Barack\ Obama,V=1961|Q=q_1,A=a_1)=1$ in Sec~\ref{sec:noise:value}.
%\end{example}
%
%\begin{center}
%\begin{tabular}{ c | c | c | c | c}
%\hline
%question & answer & entity & value & probability \\ \hline
%\hline
%$q_1$ & $a_1$ & Barack Obama & 1961 & 0.5 \\ \hline
%$q_1$ & $a_1$ & Barack Obama & politician & 0.5 \\ \hline
%\end{tabular}
%\captionof{table}{$P(E,V|Q=q_1,A=a_1)$}
%\label{tab:qaevp}
%\end{center}


%\subsection{Entity Recognition for QA Pairs}
%\label{sec:noise:ner}
%Entity detection is a fundamental block of our QA system. In Algorithm~\ref{alg:ala}, we use entity detection in both online procedure and offline procedure for new questions and questions in QA corpora, respectively. Unfortunately, current entity detection approaches are usually developed for one specific domain and cannot perform well enough on other domains~\cite{poibeau2001proper}. The problem is more striking when a large scale open domain knowledge base is used. Because, more entity candidates can be found in such a knowledge base.
%As an example, for the question ``When was Barack Obama born?'', we know that ''Barack Obama'' is a person and is the unique named entity in the question. But (1) ``Barack Obama'' can also be a name of a book in the knowledge base and (2) ``born'' can also be an entity in our knowledge base (a town in the Netherlands).
%
%Fortunately, we have a great chance to improve the accuracy of entity detection in QA corpora. Given the QA corpora, we can use the answer of a question to filter noisy entities. Continue the previous example, suppose the answer ``1961'' is in the QA corpora. The knowledge base (as shown in Figure~\ref{fig:barackobama}) tells us that  ``1961'' is exactly the birth date of node $a$ (denoting Barack Obama). In contrast, we can not find any connection between ``1961'' and ``born'' from the knowledge base. Hence, we can infer that ``Barack Obama'' is of high probability to be an entity.
%
%\paragraph*{Problem model}
%Before we formalize the problem, we present how we identify all candidate entities in the question $q$. The identification is straightforward: if an entity's name $s_1$ occurs as a substring of $q$ (denoted by $s_1\in q$), we regard it as a candidate entity. We denote this candidate entity set as $E_c$:
%$$E_c(q)=\{e| \exists s_1 \in q, (e,name,s_1) \in \mathcal{K} \}$$
%
%
%Given $E_c(q)$ for a question $q$, we define the problem model in Definition~\ref{def:er}. The key of the problem model is to define the scoring function \emph{confidence}, which in turn is based on {\it relatedness} function.
%
%\begin{definition}
%Given a QA pair $(q, a)$ and a RDF knowledge base $\mathcal{K}$, find the entity $e\in E_c$ maximizing $confidence(e)$, i.e.,
%$$\argmax_{e}confidence(e)$$, where $confidence(e)$ is a scoring function defined on $e$.
%\label{def:er}
%\end{definition}
%
%Given an answer $a$, if a substring $v\in a$ is an object in $\mathcal{K}$, $v$ is a candidate value. Let $V_c(a)$ be the set of all candidate value for the answer $a$.
%Then, for each candidate entity $e \in E_c(q)$ and each candidate value $v\in V_c(a)$ we define the \emph{relatedness} between $e$ and a substring $v$ as:
%
%\begin{equation}
%{relatedness}(e,v)=\exp(-min\{p^+.length| (e,p^+,v) \in \mathcal{K}^+\}).
%\end{equation}
%
%The relatedness score is negatively correlated with the length of $p^+$. This is because in general simpler is better. Shorter predicate is of higher probability being a meaningful predicate and more related to the entity. We further define the $confidence$ of a candidate entity $e$ as the sum of the relatedness:
%
%\begin{equation}
%{confidence}(e)=\Sigma_{v \in V_c}relatedness(e,v).
%\end{equation}
%
%%Instead of finding the entity directly from the question, we first find a string as candidate value $v$ from the answer. Then, if there exists an entity $e \in q$ and $p^+ \in \mathcal{QA}_{p^+}$ such that $(e, p^+, v) \in \mathcal{K}$, it means that the answer contains one value $v$ of candidate entity $e$ in question. This is a strong evidence that, the entity $e$ is the entity in the question. Therefore we can recognize the entity $e$.
%%
%%Using the method above, we can do the NER using Algorithm~\ref{alg:fpatkb}:
%%
%%\begin{algorithm}[h]
%%\small
%% \caption{NER for QA pair}
%%\begin{algorithmic}[1]
%%\Require{$(q,a),\mathcal{K}$;}
%%\Ensure{entities of $q$};
%%    \State {$E \leftarrow \emptyset$}
%%    \For {all substring $s_1$ of $q$}
%%        \For {all $e$ satisfy $(e,name,s_1) \in \mathcal{K}$}
%%            \For {all substring $s_2$ of $a$}
%%                \If {$\exists p^+, (e,p^+,s_2) \in \mathcal{K}$ \label{line:exists}}
%%                    \Return $E \leftarrow E \cup \{e\}$
%%                \EndIf
%%            \EndFor
%%        \EndFor
%%    \EndFor
%%    \State {\Return $E$}
%%\end{algorithmic}
%%   \label{alg:fpatkb}
%%\end{algorithm}
%
%\paragraph*{Solution}
%Given a QA pair $(q, a)$, we solve entity detection using three steps:
%\begin{enumerate}
%\item Find all candidate entities $E_c(q)$ from the question $q$.
%\item Find all candidate values  $V_c(a)$ from the answer $a$.
%\item Enumerate all $(e,v)$ pairs and sum up the {\it relatedness} to compute $confidence(e)$.
%\end{enumerate}
%Specifically, let $|q|$ be the length of the question, and $l_{q}$ be the length of the longest entity name in the knowledge base. Finding $E_c$ needs $O(|q|l_{q})$ times. Because we need to enumerate each substring of $q$ with length $\le l_{q}$, and checking whether a substring is a name in the knowledge base takes constant time if a hash index is used. Similarly, let $|a|$ be the length of the answer, and $l_{a}$ be the length of the longest value in the knowledge base, the enumeration of all candidate values takes $O(l_{v}|a|)$ times. For each $e\in E_c(q)$ and each $v\in V_c(a)$ we need to enumerate all $(e,v)$ pairs. Hence, overall it takes $O(l_q|q|+l_a|a|+|V_c(a)|E_c(q)|)$ times.
%
%Since we only need the most confident candidate entity, we can further reduce the computation cost while enumerating. The basic idea is, if we add all the possible relatedness to an entity but it still cannot has maximal confidence, we can filter this entity in further enumeration. The specific implementation is shown in Algorithm~\ref{alg:enumeration}.
%
%
%\begin{algorithm}[h]
%\small
%  \caption{Enumeration of $(e,v)$ Pairs}
%\begin{algorithmic}[1]
%\Require{$V_c$, $answer$, $E_c$, $k$}
%\Ensure{$e$}
%
%\For {all $v \in U$}
%    \State {$maxLeft+=\exp(-i)$}
%\EndFor
%\State {$maxCon=0$}
%\For {all $v \in U$}
%    \State {$maxLeft-=\exp(-i)$}
%    \For {all $e \in E_c$}
%        \If {$\exists p^+, (e,p^+,v) \in \mathcal{K^+}$ \label{line:enumeration:1}}
%            \State {$confidence(e) += relatedness(e,v)$}
%            \If {$confidence(e)>maxCon$}
%                \State {$maxCon=confidence(e)$}
%            \EndIf
%        \ElsIf {$confidence(e) +maxLeft < maxCon$}
%            \State {$E_c -= \{e\}$}
%        \EndIf
%    \EndFor
%\EndFor
%\Return {$\argmax_e Confidence(e)$}
%\end{algorithmic}
%\label{alg:enumeration}
%\end{algorithm}
%
%\paragraph*{Breaking the deadlock}
%%\reviseyh{This paragraph is not clear? How to enumerate $s_2$? what is the complexity. It seems your solution is high complexity}
%Note that, in Line~\ref{line:enumeration:1} of Algorithm~\ref{alg:enumeration},
%%in Line~\ref{line:exists} of Algorithm~\ref{alg:fpatkb},
%we need to find a shortest predicate connecting a candidate entity $e$ and a candidate value $v$. This is achieved by predicate expansion. However, predicate expansion has a prerequisite that all entities in the questions of QA corpora need to be pre-identified. In other words, entity recognition from questions implies a logic deadlock. To break the deadlock, we use $E_s^*$
%$$E_s^* = \{ e| \exists (q,a) \in \mathcal{QA}, s_1 \in a, (e,name,s_1) \in \mathcal{K} \}.$$
%as the input of predicate expansion instead of the direct $E_s$. The result of the expanded predicates in turn is used in line 8 of Algorithm~\ref{alg:enumeration} to find all entities from questions in QA corpora.


%In this algorithm, we scan the $\mathcal{QA}$. In line~\ref{alg:fpatkb:einq}, we say one candidate entity $ent \in que \iff ent$ is one substring of $que$, and $ent$ is one entity in the knowledge base. This work is supported by the Entity Indexer in Sec~\ref{sec:architecture:indexer}. We will further illustrate how we decide whether $(e,r,v) \in k$ in Sec~\ref{sec:amatomy:mapper:relation}.

\nop{
\subsection{Corpora Cleaning}
\label{sec:noise:template}
The QA corpora are crawled from Yahoo! Answer, which as an open Web data source inherently has many noises. As a result, many questions are meaningless to train our QA models. In this section, we present our method for cleaning the corpora data. We randomly select 100 question templates. We find that 53\% of templates are meaningless. These templates can be classified into three major categories as shown in Table~\ref{tab:categoryNotation}. These three categories account for the 92\% of all cases meaningless cases.


\begin{table}[!htb]
\begin{center}
\begin{tabular}{ | p{1.5cm} | l |p{1cm}|}
  \hline
  Notation & Example  & ratio \\ \hline
  \hline
  meaningful templates & how many people live in \$country & 47\% \\ \hline
  incomplete description  & what kind of \$animal be this & 12\% \\ \hline
  subjective template & what is best \$artist song & 31\% \\ \hline
  prediction & who will win \$game& 6\% \\  \hline
  others &  & 4\% \\ \hline
\end{tabular}
\caption{Category information for 53 meaningless templates}
\label{tab:categoryNotation}
\end{center}
\end{table}

The {\it prediction} questions clearly can not be answered by any knowledge base.
The {\it subjective} questions depends on repliers. These question have no unique answers and cannot be answered by a knowledge base.
The \emph{incomplete} question means that the question itself is incomplete and consequently cannot be understood by a real person. This is caused by the input format of Yahoo! Answer. We a user submit a question to Yahoo! Answer. They need to specify question title and question description. Users may submit other material such as a file, an image as a detailed description for the question. For example, a user many pose a question \emph{what kind of dog be this} and specify a picture of a dog as the description.
This kind of question and answer pairs can only be understood by real persons but hardly for a machine.

%Due to the statistics, the main noise is from \emph{incomplete description}, \emph{subjective template} and \emph{prediction}.

We use feature words to filter out these three meaningless templates:
\begin{itemize}
\setlength{\itemsep}{-1pt}
\item \emph{Incomplete questions:} most such questions contains \emph{this} or \emph{that}, because \emph{this} or \emph{that} always refers to the content the question description.
\item \emph{Subjective question:} most such questions contains subjective words, such as \emph{best}, \emph{good}, \emph{I}, and \emph{My}.
\item \emph{prediction:} most such questions contains \emph{will}, \emph{gonna}.
\end{itemize}
Given these feature words, we treat the questions as a bag of words. Any question that can be classified into one of the above category will be dropped off.

%After such filtering, these questions, which is not asking about a common knowledge, has already been filtered. But there are still many questions we cannot use directly. Because for many question, although the answer is in the knowledge base, it's not a binary factoid question. That is, the relation of the question has complex dependencies, or the relation cannot be presented by a path in the knowledge base. These questions is still meaningful for us, that we may expect solving these questions in our future work. But currently, our system still cannot answer them. So we also would like to filter them. To filter them, we also use bag-of-words model like before. More results will be presented in the experiments part.
}

\subsubsection{Entity\&Value Refinement}
\label{sec:noise:value}
In this subsection, we refine valid entity\&value pairs, i.e., the computation of $V(q,a)$ in Eq~\ref{eqn:vqa}.
% based on the work in Sec~\ref{sec:noise:jointprobability}. Due to Eq.~(\ref{eqn:vc}),
In general, multiple candidate values may exist for a given answer. In Example~\ref{example:vqa}, $(Barack\ Obama, politician)$ is an incorrect entity\&value pair for $(q_1,a_1)$. We need to filter such incorrect pairs for more accurate entity\&value recognition. %This fact motivates us to carefully identify the real $V(e,a)$.

The intuition of our refinement is: {\it the correct value and the question should have the same category.} For example, since $q_1$ is asking about {\it date}, we should not consider {\it politician} as a candidate value since it's not a date. The key to such refinement is to compute the value category and question category. And only the matching values are reserved in $V(q,a)$.

We use the UIUC taxonomy~\cite{li2002learning} in categorization. For question categorization, we use the approach proposed in~\cite{metzler2005analysis}. For value's categorization, we first find the predicate leading to this value, and then use the predicate's category. The predicate's category is from manual labeling. There are only a few thousand predicates that  this is doable.

%We introduce such category based refinement as follows: we first get the questions' category (such as date or location) by question classification~\cite{metzler2005analysis}. Then we check whether each value in the candidate value set to see whether it has the same category. If not, we remove it from the candidate set. To get a value's category, we use the categories of the predicate leading to this value. We manually labeled category for predicates with length 1. For $p^+$ that leads to the value, we set its category as follows:
%\begin{enumerate}\setlength{\itemsep}{-2pt}
%\item When $p^+$ ends with $name$, we use the category of $name$'s immediately prior predicate.
%\item When $p^+$ doesn't end with $name$, we directly use the category of $p^+$'s last predicate.
%\end{enumerate}

%\begin{example}[Value Refinement]
% For example, for ``Michelle Obama'' in the triple $(a, marriage\rightarrow person\rightarrow name, Michelle\ Obama)$,  $person$ is the last predicate and immediately prior predicate of $name$. And the category of predicate $person$ is $\#person$. Thus, the category of value ``Michelle Obama'' is $\#person$. For example, for 1961 in $(a,dob,1961)$, the last predicate is $dob$. From the labeled predicates, we know that the category of $dob$ is date. Hence, the category of ``1961'' is $\#date$.
%\end{example}


%As shown in the Example~\ref{exam:jointprobability}, the category of the question is date and only ``1961'' matches the question.
%We use question categorization and value categorization for the match.
%We directly use the classification approaches proposed for fact-based questions~\cite{metzler2005analysis} to classify our questions. The accuracy was reported to be over 90\%.


\begin{example}[Refinement]
\vspace{-0.2cm}
Continue Example~\ref{example:vqa}.
From question classification, we know the question's category is {\it date}.
%Consider the question ``When was Barack Obama born?'', and its answer ''The politician was born in 1961''.
For two candidate values: politician and 1961, their leading predicates are \emph{category} and \emph{dob}, respectively. So we know ``category'''s category is {\it desc} and ``dob'''s category is {\it date}. Therefore only the correct entity\&value pair left. So we have: $V(q_1,a_1) =\{Barack\ Obama, 1961\}$, $P(Barack\ Obama,$ $1961|(q_1,a_1))=1$.
%Both predicates do not end with $name$. Therefore we directly use the categories of them as the values' categories. The categories of \emph{category} and \emph{dob} are description and date, respectively. So the categories of ``politician'' and ``1961'' are also description and date, respectively.
%Given the entity $a$ ($\bar{a}=``Barack\ Obama''$), we know that $politician$'s predicate is $category$ and 1961's predicate is $dob$. By predicate classification, we know that the category of ``1961'' is \emph{\#date}, while the category of ``politician'' is not.
%By question categorization, we know that the category of the $q_1$ is date. Therefore ``1961'' is the only valid candidate value and we can prune ``politician''. Thus we finally have the correct probability: $P(E=Barack\ Obama,V=1961|Q=q_1,A=a_1)=1$.
\end{example}
%\begin{example}
%\label{exam:qc}
%Figure~\ref{fig:example_qc} illustrates a QA pair. The answer contains three property values about \emph{Barack Obama}: his wife ($marriage \rightarrow person \rightarrow name$, his date of marriage ($marriage \rightarrow date$),  and his place of marriage ($marriage \rightarrow location$). Clearly, only his wife name should be returned as the answer value.
%\end{example}
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.5]{figs/example_QuestionClassification.eps}
%\caption{Example for Value Extraction}
%\label{fig:example_qc} %% label for entire figure
%\end{figure}

%We use the predicate that leading to the value to do value categorization.
%Specifically, for a value $v$ in the triple $(e,p^+,v)$, the category of $p^+$ is the category of $v$. We first labeled the category for all single predicates (i.e., $p^+.length=1$) in the knowledge base. Then for an expanded predicate $p^+$ There are two cases need to be addressed:
%\begin{itemize}
%\item First, $p^+$ ends with predicate $name$. We use the name of the predicate that is immediately prior to the $name$ predicate. For example, for ``Michelle Obama'' in the triple $(a,marriage\rightarrow~person\rightarrow~name, Michelle\ Obama)$,  $person$ is the immediately prior predicate of $name$. And the category of predicate $person$ is $\#person$. Thus, the category of value ``Michelle Obama'' is $\#person$.
%\item Second, $p^+$ doesn't end with $name$. We directly use the category of $p^+$'s last predicate as the value's category. For example, for 1961 in $(a,dob,1961)$, the last predicate is $dob$. From the labeled predicates, we know that the category of $dob$ is date. Hence, the category of ``1961'' is $\#date$.
%\end{itemize}
%The syntactic feature it use for a question, is the \emph{bigram}. It is possible to achieve reasonable results using syntactic features alone, except for \emph{what} questions. For what questions, we use the category of the first noun phrase as the feature. For example, for the question \emph{what is the capital of China}, \emph{capital} is the first noun. And knowing that \emph{capital} is a location allow us to assign the correct type. We use POS tagger of Senna~\cite{collobert2011deep} to find the first noun phrase. To train the classifier for noun, we use 5500 labeled questions from TREC~\footnote{http://cogcomp.cs.illinois.edu/Data/QA/QC/}. The author of~\cite{metzler2005analysis} claimed that this simple strategy can achieve the accuracy of

